Learning Shared Semantic Space for Speech-to-Text Translation

Having numerous potential applications and great impact, end-to-end speech translation (ST) has long been treated as an independent task, failing to fully draw strength from the rapid advances of its sibling - text machine translation (MT). With text and audio inputs represented differently, the modality gap has rendered MT data and its end-to-end models incompatible with their ST counterparts. In observation of this obstacle, we propose to bridge this representation gap with Chimera. By projecting audio and text features to a common semantic representation, Chimera unifies MT and ST tasks and boosts the performance on ST benchmarks, MuST-C and Augmented Librispeech, to a new state-of-the-art. Specifically, Chimera obtains 27.1 BLEU on MuST-C EN-DE, improving the SOTA by a +1.9 BLEU margin. Further experimental analyses demonstrate that the shared semantic space indeed conveys common knowledge between these two tasks and thus paves a new way for augmenting training resources across modalities. Code, data, and resources are available at https://github.com/Glaciohound/Chimera-ST.

==> arxiv submission v3/body/000abstract.tex <==

Having numerous potential applications and great impact, end-to-end speech translation (ST) has long been treated as an independent task, failing to fully draw strength from the rapid advances of its sibling - text machine translation (MT). With text and audio inputs represented differently, the modality gap has rendered MT data and its end-to-end models incompatible with their ST counterparts.
In observation of this obstacle, we propose to bridge this representation gap with \model.
% (\modelfullname).
%\heng{I'm not sure if you are allowed to change abstract after the abstract deadline. pls double check.} 
By projecting audio and text features to a common semantic representation, \model unifies MT and ST tasks and boosts the performance on ST benchmarks, MuST-C and Augmented Librispeech, to a new state-of-the-art. Specifically, \model obtains 27.1 BLEU on MuST-C EN-DE, improving the SOTA by a +1.9 BLEU margin.
Further experimental analyses demonstrate that the \method indeed conveys common knowledge between these two tasks and thus paves a new way for augmenting training resources across modalities.
Code, data, and resources are available at \url{https://github.com/Glaciohound/Chimera-ST}.

==> arxiv submission v3/body/010intro.tex <==

Speech-to-text translation (ST) takes speech input in a source language and outputs text utterance in a target language. It has many real-world applications, including automatic video captioning, simultaneous translation for international conferences, etc.
Traditional ST approaches cascade automatic  speech recognition (ASR) and machine translation (MT)~\cite{sperber2017neural,sperber2019self,zhang2019lattice,beck2019neural,cheng2019breaking}.
However, cascaded models often suffer from the issues of error propagation and translation latency.
As a result, there have been a series of recent attempts on end-to-end speech-to-text translation ~\citep{liu2019end, liu2018ustc, weiss2017sequence, berard2018end, duong2016attentional, jia2019leveraging,dong2021listen, wang2020curriculum}. The end-to-end approaches learn a single unified model, which is easier to deploy, has lower latency and could potentially reduce errors.

However, it remains a challenge for end-to-end ST to catch up with their cascaded counterparts in performance. We argue that the root cause is the gap between the two modalities, speech and text.
Although they both encode human languages, they are dissimilar in both coding attributes (pitch, volume, and intonation versus words, affixes, and punctuation)
and length (thousands of time frames versus tens of words). This issue is further coupled with the relatively smaller amount of parallel data for ST than for MT.

% ~\citep{sperber2017neural, sperber2019self, zhang2019lattice, beck2019neural,  cheng2019breaking}.
% One source of power of the cascaded approach is that it can incorporate a large amount of ASR and MT data, and train its two corresponding sub-modules separately. Traditional yet still effective, the now stagnated success of cascaded ST sheds light on how end-to-end models could improve themselves by making use of additional sources of data.
% \heng{I think this whole paragraph needs to be re-organized. The story should be like this: (1) Existing successful methods use cascaded model because they can take advantage of the text-to-text translation training data; (2) But cascaded model shave disadvantages: efficiency, error propagation, ... (3) So we aim to train end-to-end model; but existing methods still cannot outperform cascaded model because it cannot leverage existing text to text translation resources due to the modality gap. (4) so we propose a new share semantics space between speech and text to fill in the gap... }
% \hanchi{will do}

To tackle these challenges, we resort to making use of the additional available bilingual data for MT.
Our hypothesis is, to better leverage MT data,
an ideal model should be able to bridge the representations between speech and text.
Motivated by this intuition, we propose \model, a \modelfullname. It learns a \methodrepresentation by projecting features from both modalities into a \method.
% \model consists of a unified architecture with an encoding module, a \methodprojection module, and a decoding module. 
% This approach has the advantage of unifying ST and MT tasks and can leverage massive MT training corpora as a side boost in training.
This approach unifies ST and MT workflows and thus has the advantage of leveraging massive MT corpora as a side boost in training. It can also use speech-text pairs to align the \methodrepresentations from two modalities.

\cameraready{
This idea of a unified text-speech representation also finds its neural basis as suggested by recent evidence from functional neuroimaging
~\citep{vanatteveldt2004271, spitsyna2006converging, shankweiler2008reading}.
Specifically, ~\citet{vanatteveldt2004271, spitsyna2006converging} identifies certain regions in brain that the processing stream for speech sounds and visual texts converge at.
% , such as those in superior temporal sulcus (STS) and the parietal-temporal-occipital (PTO) junction. 
~\citet{shankweiler2008reading} further verifies that the size of such convergence sites correlates positively with the subjects' reading skills.
Coincidentally, at these convergence sites also found regions responsive to downstream activities such as lexical and semantical word recognition ~\citep{binder2003neural} and spontaneous generation of speech ~\citep{blank2002speech}. The evidence establishes the pivotal role of a modality-agnostic converged representation in language activities in brain.
% Specifically, ~\citet{vanatteveldt2004271} locates several regions in superior temporal sulcus (STS) in human brain which respond to both speech and text signals.
% When presented together, the signals are boosted, and even early speech responses in planum temporale/Heschl's sulcus (PT/HS) can be modulated by text, a phenomenon named letter-speech sound (LSS) integration.
% It also proves simultaneously presented texts can even modify speech representations, based on whether contents are congruent or not.
% Later studies show that the childhood acquisition of reading skills is accompanied with learning LSS integration ~\citep{Froyen2009longroad}, which further appears to play a critical role in reading fluency because children dyslexia (a type of reading disorder) is associated with inability to acquire such integration ~\citep{Froyen2011EvidenceFA}.

This intuition lacks exploration in previous studies, with only a few exceptions ~\citep{indurthi2020data, liu2020bridging}, possibly due to the difficulties aforementioned and marginal improvements.}

% Our experiments compare \model against several neural baselines. 
Our results show that \model achieves new state-of-the-art results on all of 8 translation directions in the benchmark datasets MuST-C and Augmented LibriSpeech.
Specifically, \model obtains a 27.1 BLEU score on MuST-C EN-DE, which surpasses the best result ever reported by up to +1.9 BLEU. 
We also provide results under variations and ablations and validate our model design ideas by detailed analysis, as well as visualizing the semantic space \model has learned.
% The visualization shows that \model is capable of learning a modality-agnostic and well-structured shared semantic space for text and speech. 

Our work makes the following contributions.
First, we propose \model, which is able to bridge the modality gap between speech and text. Second, we derive a novel bi-modal contrastive training task to learn an alignment between \methodrepresentations of two modalities. Finally, \model achieves a new state-of-the-art performance on the MuST-C benchmark and demonstrates its efficacy in learning modality-agnostic semantic representations.
% through a series of ablation studies and visualizations.

==> arxiv submission v3/body/020related.tex <==

\noindent\textbf{End-to-end ST}~
Since its first proof-of-concept work \citep{berard2016listen, duong2016attentional}, solving Speech Translation in an end-to-end manner has attracted extensive attention ~\citep{vila2018end, salesky2018towards, salesky2019fluent, di2019adapting, bahar2019comparative, di2019enhancing, inaguma2020espnet}.
Standard training techniques such as pretraining ~\citep{weiss2017sequence, berard2018end, bansal2019pre, stoian2020analyzing, wang2020bridging, pino2020self}, multi-task training ~\citep{vydana2021jointly, le2020dual, tang2021general}, meta-learning ~\citep{indurthi2020data}, and curriculum learning ~\citep{kano2018structured, wang2020curriculum} have been applied.
% to ST models to improve performance. 
As ST data are expensive to collect, ~\citet{jia2019leveraging, pino2019harnessing, bahar2019using} augment synthesized data from ASR and MT corpora. Methods utilizing trained models, such as knowledge distillation ~\citep{liu2019end} and model adaptation ~\citep{di2020instance}, have also been shown to be effective.
Among these attempts, \cite{indurthi2020data, le2020dual, liu2020bridging}
are most related to ours, as they also attempt to train models on ASR or MT data. However, they both lack pivotal modules in model design to semantically bridge the gap between audio and text, and could thus suffer from modality mismatch in representations.


\noindent\textbf{Cascaded ST}~
The cascaded method is a more long-standing trend in ST
% , which works by applying ASR (audio $\rightarrow$ transcript) and MT (transcript $\rightarrow$ translation) successively 
~\citep{sperber2017neural, jan2018iwslt}.
To alleviate its innate problem of error propagation, ~\citet{cheng2018towards, cheng2019breaking} introduce synthetic ASR-related errors and perturbations. On the other hand, some post-processing techniques such as re-segmentation ~\citep{matusov2006automatic}, punctuation restoration ~\citep{fugen2008system}, and disfluency detection ~\citep{fitzgerald2009reconstructing}
are proposed to fix flaws or errors that occurred during the translation.
% ~\citet{liu2003use, fugen2008system} also used domain-adaptation to better train a cascaded model.

\cameraready{
\noindent\textbf{Cross-Lingual Techniques}~
Techniques in multilingual tasks is also related to ours, as they aim at extracting common features out of sources from different representations (which, in this case, is language diversity) as well. However, multilingualism lacks key difficulties as observed in audio-text modality gap as discussed before.
~\cite{lu2018neural} and ~\cite{vazquez2019multilingual} are early attempts by building an LSTM-based attentional interlingua. ~\citet{yu2018multilingual, yang2019improving} uses a similar cosine-based loss for multilingual training. ~\citet{zhu2020language} is probably more similar in method to ours, but \model is more simple in terms of model and objectives, and the memories in \model are additionally designed to focus on specific semantic categories.
}

==> arxiv submission v3/body/030method.tex <==

% This section presents the overall setting of the problem and then introduce the framework of the proposed \model and its training objectives.

\input{body/031overview}
\input{body/032sharedmem}
\input{body/033obj}

==> arxiv submission v3/body/031overview.tex <==

\subsection{Speech Translation Overview}
\label{subsec:overview}

An ST corpus usually consists of a set of triplet data \(\mathcal{S}=\{(\mathbf{x}_i, \mathbf{z}_i, \mathbf{y}_i)\}\). Here \(\mathbf{x}_i\) is the audio wave sequence, \(\mathbf{z}_i\) is the transcript sequence and \(\mathbf{y}_i\) is the translation sequence in the target language.
As a benefit of \methodprojection, \model is able to leverage large-scale MT training corpora \(\mathcal{T}=\{(\mathbf{u}_i, \mathbf{v}_i)\}\), where \(\mathbf{u}_i\) and \(\mathbf{v}_i\) are the source and target text sequences.

% Traditionally, the input $\mathbf{x}$ is processed into Mel-Frequency Cepstral Coefficients (MFCCs) as raw features. However, the recent Wav2Vec2 ~\citep{baevski2020wav2vec} method introduces a self-supervised feature trained on raw audio waves, much similar to the role of BERT in natural language text. This forms the basic audio feature extractor of our model.

==> arxiv submission v3/body/032sharedmem.tex <==
\subsection{\model Architecture}
\label{subsec:memory}

Figure \ref{fig:method} illustrates the structure of \model. It consists of three major components, an encoding module, a \methodprojection module, and a decoding module. 

\noindent\textbf{Encoding Module} 
Different from that of a conventional ST model, the encoding module of \model accepts either speech or text as input. For text input, we use word embeddings plus positional embeddings. For speech input, we use a pretrained Wav2Vec2 ~\citep{baevski2020wav2vec} to extract speech features. As the speech features can be very long, we apply an additional 1-dimensional strided CNN to reduce the length.
Both speech and text branches share a common subsequent Transformer encoder ~\citep{vaswani2017attention}. The final output of the encoding module is contextual features.
% $\mathbf{E}(\mathbf{x})$ or $\mathbf{E}(\mathbf{u})$, where $\mathbf{x}$ comes from ST corpus $\mathcal{S}$ and $\mathbf{u}$ comes from MT corpus $\mathcal{T}$.


\noindent\textbf{\MethodProjection Module}
\Methodprojection plays a pivotal role in \model. The contextual features of speech and text may follow different distributions and of different lengths.
% The length of $\mathbf{x}$ is also much larger than that of $\mathbf{u}$.
Ideally, the \methodprojection computes a constant number of semantic features as its output \methodrepresentations. 
% Ideally, the features should only contain information necessary for downstream decoding, regardless of the difference between speech and text. As a result, we design this module to map the inputs with different lengths to a shared and fixed-size representation.

This module take the contextual features out from the encoding module as input and then output \methodrepresentations of fixed length $m$. It consists of $n$ attentional layers.
% It keeps a tuple of $m$ trainable \methodembeddings to indicate the types of desired semantic information. A concatenation of contextual features and \methodembeddings along the sequence dimension is fed into \methodprojection, which consists of $n$ iterations of Transformer-like projection layers. In each projection layer, the input is passed through a multi-head attention network, a layer-norm, and a feed-forward network, and then stripped off the starting part to keep only the last $m$ elements. These elements are the output of this projection layer. They are concatenated with contextual features again and fed into the next projection layer. Note that the output of each projection layer has the same length $m$. The final output is used as the \methodrepresentation.
It keeps a tuple of $m$ trainable input-dependent \methodembeddings to indicate the types of desired semantic information, which is used as the initial ``memories''. Uni-modal contextual features serves as attention ``keys'' and ``values'', while memories serves as attention ``queries``. Memories are iteratively fed to the $n$ \methodprojection layers, with each layer output used as input to next layer. The final output is used as the \methodrepresentation.

\begin{gather}
% \mathbf{I}_0 = \text{concatenate}(\mathbf{\hat{H}}, \mathbf{M}_0) \in \mathbb{R}^{(l+m)\times d} \\
\mathbf{I}_0 = \mathbf{M}_0
\in \mathbb{R}^{m \times d}
\\
\mathbf{K}_i = \mathbf{V}_i = \mathbf{\hat{H}}
\in \mathbb{R}^{l\times d}
\\
\mathbf{I}_{i+1} = \mathbf{O}_i = \text{Attn}(\mathbf{I}_i, \mathbf{K}_i, \mathbf{V}_i)
\in \mathbb{R}^{m \times d}
% \\
% \mathbf{I}_{i+1} \noindent\textbf= \text{concat}(\mathbf{\hat{H}}, \mathbf{O}_i)
% \in \mathbb{R}^{(l+m)\times d}
\end{gather}
where $\mathbf{M}_0$, $\mathbf{\hat{H}}$, $\mathbf{I}_i$ and $\mathbf{O}_i$ denote the \methodembeddings, contextual features, the input, and the output of each layer, respectively. $l$ is the length of contextual features. $d$ is the shared vector dimension. The top-most output $\mathbf{O}_n$ is finally fed into the decoding module. 

\noindent\textbf{Decoding Module}
The decoding module contains a conventional Transformer decoder. The only difference is that the input is the fixed-size $\mathbf{O}_n$, which can possibly come from either speech or text.

==> arxiv submission v3/body/033obj.tex <==
\subsection{Training Objectives}
\label{subsec:obj}
The training objective of \model consists of three aspects, with their supervision signals coming from speech-to-text translation data $\{(\mathbf{x}_i, \mathbf{y}_i)\}$, text machine translation data $(\{\mathbf{u}_j, \mathbf{v}_j)\}$ and $(\{\mathbf{z}_i, \mathbf{y}_i)\}$ and the speech-transcript pairs $\{(\mathbf{x}_i, \mathbf{z}_i)\}$. 

% \noindent\textbf{Speech-to-Text Translation Training}
\noindent\textbf{Speech-to-Text Translation Training}
The workflow of \model in Speech Translation is straightforward. The training objective is
% After the encoding module gets contextual features from the audio wave $\mathbf{x}$, the \methodprojection module is responsible for projecting them into the \method as \methodrepresentation. Finally, the decoder module outputs the target translation based on \methodrepresentation. 
% This training objective is exactly the same as conventional end-to-end speech translation models,
negative log-likelihood on speech-to-text translation data $\{(\mathbf{x}_i, \mathbf{y}_i)\}$ from the data $S$ as the loss function.
\begin{equation} \label{eq:ST}
% \mathcal{L}_\text{ST} = - \mathbb{E}_{\mathbf{x},\mathbf{y}}{
%     \log \text{Pr}_{
%         \mathbf{\hat{y}} \sim \mathbf{D}(\mathbf{P}(\mathbf{E}(\mathbf{x})))
%     } (\mathbf{\hat{y}} = \mathbf{y})
% }
\mathcal{L}_\text{ST} = - \mathbb{E}_{\langle\mathbf{x},\cdot,\mathbf{y}\rangle \in \mathcal{S}} \log P (\mathbf{y} | \mathbf{x})
\end{equation}
% \rong{Simple notation: $- \mathbb{E}_{\mathbf{x},\mathbf{y}} \log \text{P} (\mathbf{y} | \mathbf{x})$ is ok. }

\noindent\textbf{Text Machine Translation Training}
% The speech translation training objective is powerful enough to make full use of machine translation training data $(\mathbf{u}, \mathbf{v})$. 
\model is also able to train on parallel sentences because of the unification of speech and text representations.
%, as well as the unification of ST and MT tasks in the workflow. 
The parallel data are directly from MT dataset or transcript-translation pairs.
This enables the model to further acquire knowledge from the much larger extra MT corpus. 
% In MT training, the input data flows through the text branch of the model. 
Similar to ST training, the \methodprojection module projects the contextual text features to the \method, which are then taken by the decoding module to output a translation.
\begin{equation} \label{eq:MT}
% \mathcal{L}_\text{MT} = - \mathbb{E}_{\mathbf{u},\mathbf{v}}{
%     \log \text{Pr}_{
%         \mathbf{\hat{v}} \sim \mathbf{D}(\mathbf{P}(\mathbf{E}(\mathbf{u})))
%     } (\mathbf{\hat{v}} = \mathbf{v})
% }
\begin{aligned}
\mathcal{L}_\text{MT} = & - \mathbb{E}_{ \langle\cdot, \mathbf{z},\mathbf{y} \rangle \in \mathcal{S} } \log P (\mathbf{y} | \mathbf{z}) \\ 
& - \mathbb{E}_{\langle\mathbf{u},\mathbf{v} \rangle \in \mathcal{T}   } \log P (\mathbf{v} | \mathbf{u})
\end{aligned}
\end{equation}

\noindent\textbf{Bi-modal Contrastive Training}
The motivation of \model design is to bridge the speech and text representations.
% It is then natural to incorporate the parallel speech-transcript data $\{(\mathbf{x}_i, \mathbf{z}_i)\}$ as training supervision. 
We introduce dual-modal contrastive training to learn an alignment between representations from speech and text as illustrated in Figure \ref{fig:contrastive}.
First, \methodrepresentations from two inputs are computed. Then for each text \methodrepresentation, $\mathbf{M}_i^{text}$, we compute its cosine similarities with all speech \methodrepresentation  $\{\cos(\mathbf{M}_i^{text}, \mathbf{M}_j^{speech})\}$. They are then fed into a softmax function. The loss function maximizes the item from matched pairs $(\mathbf{M}_i^{text}, \mathbf{M}_i^{speech})$. Finally, the loss is summed across all text memory items and vise versa.

% The mathematical form of the contrastive loss $\mathcal{L}_\text{ctr}$ is as follows:

\begin{equation} \label{eq:contrastive}
\begin{split}
\mathcal{L}_\text{ctr} = &- \mathbb{E}_{\mathbf{x}, \mathbf{z}} \sum_i 
    \text{ln}  \frac{e^{\tau\text{cos} (\mathbf{M}_i^\text{text},\mathbf{M}_i^\text{speech})}}{\sum_j e^{\tau\text{cos} (\mathbf{M}_i^\text{text},\mathbf{M}_j^\text{speech})}} \\
    & -
    \mathbb{E}_{\mathbf{x}, \mathbf{z}} \sum_j 
    \text{ln}  \frac{e^{\tau\text{cos} (\mathbf{M}_j^\text{speech},\mathbf{M}_j^\text{text})}}{\sum_i e^{\tau\text{cos} (\mathbf{M}_j^\text{speech},\mathbf{M}_i^\text{text})}} 
\end{split}
\end{equation}

Intuitively, the contrastive loss forces the pair $(\mathbf{M}_i^{text}, \mathbf{M}_i^{speech})$ to project \methodrepresentations close to each other.
% In the meantime, as the softmax function also minimizes the non-matched pairs, 
% \(\{(\mathbf{M}_i^{text}, \mathbf{M}_j^{speech}) \mid i \ne j\}\)
In the meantime, the softmax function trains the model to maintain diversity among \methodrepresentations.

The final loss is a weighted sum of each loss:
\begin{equation} \label{eq:loss}
\mathcal{L} =
\lambda_\text{ST} \mathcal{L}_\text{ST} +
\lambda_\text{MT} \mathcal{L}_\text{MT} +
\lambda_\text{ctr} \mathcal{L}_\text{ctr}
\end{equation}

==> arxiv submission v3/body/040exp.tex <==


We conduct experiments on the benchmark MuST-C and, as a validation of model design, carry out ablation studies and visualize the representations \model has learned.

\input{tables/main_results}
\input{tables/librispeech_results}
\input{tables/mt_baselines}

\input{body/041data}
\input{tables/freezing_modules}

\input{body/042configuration}

\input{tables/multitask}


\input{body/043benchmark}
\input{fig/mt_size}

% \rong{A concern: since you compare TS4 with the cascaded model, and TS4 uses external MT data, what if the cascaded model also uses external MT data to train the Transformer MT? Or what if wav2vec2 is used in Transformer ASR + CTC? }

\input{body/0440ablation}

==> arxiv submission v3/body/041data.tex <==

\subsection{Dataset and Preprocessing}
% \chengqi{where is "preprocessing"? word-level?BPE?}
\label{subsec:data}

\noindent\textbf{MuST-C} ~\citep{di2019must} is a multilingual speech translation corpus with triplet data sources: source audio, transcripts, and text translations. 
MuST-C contains translations from English (EN) to 8 languages: Dutch (NL), French (FR), German (DE), Italian (IT), Portuguese (PT), Romanian (RO), Russian (RU), and Spanish (ES). With each pair consisting of at least 385 hours of audio recordings, 
to the best of our knowledge, MuST-C is currently the largest speech translation dataset available for each language pair. It includes data from English TED talks with manual transcripts and translations at the sentence level. We use the dev and tst-COMMON sets as our development and test data, respectively.

\cameraready{
\noindent\textbf{Augmented LibriSpeech Dataset (En-Fr)} ~\citep{kocabiyikoglu2018augmenting} is composed of aligned e-books in French and their human reading in English.
% Aside from typical triplet data of English speech, transcript and French text, the dataset additionally provides augmented references by Google Translate.
It provides typical triplet data of English speech, transcript and French text.
Following the setting of ~\citep{liu2019end}, we utilize the 100h hours of clean train set as training data, and use the original 2 hours of dev set and and 4 hours of test set.
}

\noindent\textbf{Machine Translation Datasets} After bridging the modality gap, \model has the potential power to utilize Machine Translation resources. Therefore we incorporate data from WMT, OpenSubtitles ~\citep{lison2016opensubtitles2016} and OPUS100~\citep{zhang2020improving} translation tasks. Specifically, we use WMT 2014 ~\citep{bojar2014findings} \footnote{http://www.statmt.org/wmt14/translation-task.html} for EN-DE, EN-FR, EN-RU and EN-ES,  WMT 2016 ~\citep{bojar2016findings} \footnote{ https://www.statmt.org/wmt16/translation-task.html} for EN-RO, and OPUS100 \footnote{http://opus.nlpl.eu/opus-100.php} for EN-PT, EN-IT, and EN-NL, as pretraining corpora. We additionally evaluate OpenSubtitles as EN-DE MT data to test the impact of MT corpus selection. WMT 2014 dataset provides at least 4 million sentences of translation data in each language pair. WMT 2016 contains less, around 600k for EN-RO direction. OPUS100 has around 1M sentences for each sentence pair. OpenSubtitles provides 22M sentences for EN-DE.

\noindent\textbf{Pre-processing of Data and Evaluation}
For speech input, the 16-bit raw wave sequences are normalized by a factor of $2^{15}$ to the range of $[-1, 1)$.

For text input, on each translation pair, all texts (ST transcripts and translation, and MT source and target texts) are pre-processed in the same way. Texts are case-sensitive. Punctuation is kept, split from words, and normalized. Non-print punctuation is removed. The sentences are then tokenized with Moses tokenizer \footnote{https://github.com/moses-smt/mosesdecoder/blob/master/scripts/tokenizer/tokenizer.perl}. We filter out samples whose number of source or target tokens is over 250 and whose ratio of source and target text lengths is outside range $[ 2/3, 3/2 ]$. For sub-wording, we use a unigram sentencepiece\footnote{https://github.com/google/sentencepiece} model with a dictionary size of 10000. On each translation direction, The sentencepiece model is learned on all text data from both ST and MT corpora. The dictionary is shared across MT and ST and across source and target languages.

Unless otherwise stated, performance is evaluated with BLEU~\citep{papineni2002bleu} using sacreBLEU \footnote{https://github.com/mjpost/sacrebleu, with configuration of 13a tokenzier, case-sensitiveness and full punctuation}.
We average 7 consecutive checkpoints around the one of the best dev loss and adopt a beam size of 10. % \rong{put this in preprocessing of data and evaluation, "evaluation"  you know...}

==> arxiv submission v3/body/042configuration.tex <==

\subsection{Model Configuration}
\label{subsec:config}

For text input, we use 512-dimensional word embeddings plus sinusoidal positional embeddings.
For audio input, the Wav2Vec2 Module follows the base configuration in ~\citet{baevski2020wav2vec}. It uses parameters pretrained on LibriSpeech audio data only. The 1-dimensional CNN for speech features has 2 layers with stride size 2, kernel size 5, padding 2, and hidden dimension 1024.

The shared Transformer encoder consists of 6 layers. The \methodembeddings are 64 512-dimensional vectors. The parameters of \methodprojection resemble a 3-layer Transformer encoder. The Transformer decoder has 6 layers.
Each of these Transformer layers, except for those in the Wav2Vec2 module, has an embedding dimension of 512, a hidden dimension of 512, and 8 attention heads.

In both pretraining and fine-tuning stages, we use an Adam optimizer with $\beta_1=0.9, \beta_2=0.98$, and 4k warm-up updates. We apply an inverse square root schedule algorithm for the learning rate.
In MT pretraining, the learning rate is 5e-4, the maximum number of updates is 300k, with at most 33k input tokens per batch.
In ST pretraining, the learning rate is 1e-4, the maximum number of updates is 150k, with at most 16M source audio frames per batch.
The loss weights $\lambda_\text{ST}$, $\lambda_\text{MT}$ and $\lambda_\text{ctr}$ are all set to 1.

We also show results on a base version of \model, for which the \methodembeddings are only 16 512-dimensional vectors (codenamed ``Mem-16''). Because of the training efficiency and simplicity, all ablation studies and visualizations adopted the Mem-16 configuration if not stated otherwise. 

Both \model and \model Mem-16 contain around 165M parameters. The whole training process for one trial on 8 Nvidia Tesla-V100 GPUs generally takes 20 \textendash 40 hours according to the translation direction.


==> arxiv submission v3/body/043benchmark.tex <==
\subsection{Benchmark Experiments}
% \chengqi{I'd like to know the detailed model structure, e.g. the number of layers, the width of transformer, ...}
\label{subsec:benchmark}


\noindent\textbf{Training}
We train \model in a pretrain - fine-tune manner. 
% \rong{no need space lah! just "pretrain-finetune"}
In the first stage, we pretrain \model on MT datasets so as to leverage additional sources of training data, as well as provide a better initialization point.
% The MT data contains both external MT corpora such as WMT and OPUS100 and the transcript-translation data from MuST-C dataset.
In the fine-tuning stage, we adopt multi-task training as described in Section\ref{subsec:obj}. In addition to the conventional ST task, \model is also fine-tuned on MT and bi-modal contrastive task to align inputs from speech and text.

% We load the pretrained weights of the original Wav2Vec2 ~\citep{baevski2020wav2vec}.
% During pretraining and fine-tuning, all weights in the model are updated.
% The dictionary and unigram sub-word model are shared across pretraining and fine-tuning.

\noindent\textbf{Baselines} 
% We include both end-to-end and cascade models in our results. For cascaded models, we show the results from Espnet ~\citep{inaguma2020espnet}. For end-to-end models, 
We include as baselines the speech transformer model from~\cite{ott2019fairseq}, Espnet result from~\cite{inaguma2020espnet}, adaptive feature selection method from~\cite{zhang2020adaptive}, dual-decoder Transformer from~\cite{le2020dual} and Modality-Agnostic Meta-Learning from~\cite{indurthi2020data} in Table \ref{tab:main_results}.
% Among these baselines, ~\citet{indurthi2019data} utilize external WMT16 EN-DE and EN-FR dataset. %, which contains ~53M sentences for each language pair.
We also provide a series of baseline results of a simple combination of Wav2Vec2 ~\citep{baevski2020wav2vec} and Transformer.
It could be viewed \model without external MT pre-training, with still competitive but not SOTA results. % In this case, \methodprojection serves as nothing but additional transformer layers.

To verify the effectiveness of our training technique, we also compare with other baselines able to leverage external MT corpus in Table \ref{tab:mt_baselines}.

\noindent\textbf{Results}
The experiment results are shown in Table \ref{tab:main_results} and \ref{tab:librispeech}. Our \model achieves state-of-the-art performance on all language pairs, even though we do not utilize Google Translate results on Augmented Librispeech as most baselines. EN-DE results of \model uses WMT14+OpenSubtitles for MT pre-trainng, while a detailed ablation study on the effect of MT data can be found in Section \ref{subsec:ablation_mtdata}. Note that the improvement on EN-PT is not so significant as EN-DE and EN-FR. We attribute this to the data discrepancy between OPUS100 and MuST-C. A large number of sentences in OPUS100 are from movie subtitles, which are more informal, contain repeated sentences, and cover different topics from those in MuST-C public speeches.

In Table \ref{tab:mt_baselines}, under the same data condition, \model outperforms other techniques such as decoder pre-training and knowledge distillation ~\citep{liu2019end}.
% For example, in OPUS100 there are over 50 sentences which are simple variants of ``I can do this''. This might have limited the quality of pretrained weights at the end of MT pretraining. 
% We will prove this hypothesis in later ablation studies
% \heng{maybe in the remaining time spend time to improve results for the rest of languages. most reviewers still care about numbers a lot. If you really cannot outperform them, maybe show the size of MT pretraining data for each language pair to verify your hypothesis.}
% \hanchi{Will try}

% In later ablation experiments (Figure \ref{fig:mtdata}), we will prove this hypothesis. The results demonstrate that \model rely heavily on a large amount of high-quality data for a better performance.

% This hypothesis is partially proven by the comparison between the last two row in Table \ref{tab:main_results}. Without MT pretrainig, the performance of \model is greatly harmed when only able to learn from the ST dataset. This illustrates the importance of massive high-quality MT pretraining data for \model.

==> arxiv submission v3/body/0440ablation.tex <==
\subsection{Ablation Studies and Visualizations}
\label{subsec:ablation}

\input{fig/16memories}

\input{fig/visualization}

\input{body/0441-freezing_modules}

\input{body/0442-multitask}

\input{fig/attention_map}
\input{body/0445-mtdata}

\input{body/0446-visualization}

==> arxiv submission v3/body/0441-freezing_modules.tex <==
\paragraph{Knowledge Shared across Tasks}


One potential benefit in our design is that the \method can hold common knowledge shared across ST and MT tasks. To validate this motivating idea, we analyze the model's behavior while manipulating its modules. If certain weights pretrained during the MT task also contain meaningful information for ST, fixing them should not greatly harm the model's performance.

Specifically, after MT pretraining, we fix certain modules and do not update their weights during fine-tuning.
% As the \methodprojection Module is the first merging point for speech and text computation paths,
We choose to fix the weights in the \methodprojection module, the decoding module, or both of them.

Table \ref{tab:freezing} shows the results. After freezing modules, the results on both EN-DE and EN-FR drop slightly. This demonstrates that freezing weights indeed hampers the model's ability to adapt from MT to ST dataset. But the decreased scores are still comparable to many of the best results in Table \ref{tab:main_results}. This validates the effectiveness of \method, and indicates that the weights pretrained on MT are already informative enough for \model to still generalize sufficiently well on ST task.
% Even though the pretraining process only involves MT data, the knowledge learned in the \methodprojection module and decoding module is still highly task-agnostic. The learned common knowledge is generalizable to the ST task even if not updated during fine-tuning.

==> arxiv submission v3/body/0442-multitask.tex <==
\paragraph{Multi-task Training}

One advantage of bridging the modality gap is that the model can fully benefit from training on auxiliary tasks with more data, such as those mentioned in Section \ref{subsec:memory}.
% For example, the MT task contains information on how decoding should be done given a near perfect transcript. On the other hand, dual-modal contrastive training teaches the model to align the \methodrepresentations between speech and text inputs, which can further improve the knowledge sharing between MT and ST tasks.
% \heng{I don't understand what you mean by "draw memories"} 
% \hanchi{Oh I meant "drag two thing closer". I have changed the wording.}
To evaluate their impacts, we conduct another ablation study on EN-DE and EN-FR.. Either or both of the auxiliary tasks are not used during fine-tuning.
% , as their MT training data are the largest. We expect to observe a larger influence on these language pairs when auxiliary task are removed. For example, 
% If the \methodrepresentations are not well aligned due to the lack of contrastive loss, there will be a larger drop in the model's ability to utilize shared knowledge from MT data.

The results of this ablation are presented in Table \ref{tab:multitask}. Here we can see a significant decrease (with, for example, p=0.020 in one-tailed Student's t-test comparing row 1 and 2) in BLEU scores when either of the auxiliary tasks is abandoned. Although the bi-model contrastive loss is not directly related to the ST task, a poor alignment between \methodrepresentations of speech and text hinders \model from leveraging the shared knowledge across two tasks.
When the MT task is removed, the drop in BLEU scores is also huge.
% This could be explained as the lo of MT information transferred to ST task. 
This could be explained that during fine-tuning, the auxiliary MT task is necessary for keeping shared knowledge from being forgotten.

It is interesting to observe that abandoning both tasks produces results similar to abandoning either one of the tasks. This suggests that the two auxiliary tasks only have effects when combined with each other: only when both using MT task to maintain the pretrained parameters from forgetting, as well as using the bi-modal contrastive task to align between speech and text representations, can \model benefit from shared knowledge in MT pretraining.

==> arxiv submission v3/body/0443-memory_size.tex <==
\paragraph{\methodrepresentation Length}
% Intuitively, different \methodrepresentation lengths suit different purposes. As source texts are generally shorter than speeches (tens of sub-word tokens versus 50k~1M audio frames), longer memory contains sufficient space for information from speech, while a shorter one prevents over-fitting on MT.
Intuitively, a larger \methodrepresentation length increases the \model's expressive power. We test its effects on two choices of \methodrepresentation lengths: 16 and 64.
% \sout{redundant features}
% \heng{what do you mean by "prevents redundant features"?} 
% \hanchi{How about now?}
% when pretraining on MT. We study the model's behavior by varying the memory length to get quantitative supporting evidence for such hypotheses.
% We tested no two choices of \methodrepresentation lengths: 16 and 64, examining its influence on model performance.
The results are listed in Figure \ref{tab:memory_size}. It shows results on the MuST tst-COMMON set on EN-DE and EN-FR. ``MT'' columns show the transcript-translation BLEUs after MT pretraining. ``ST'' means the final speech translation model. A \methodrepresentation length of 16 generally results in inferior BLEUs on both MT and ST. We hypothesize that this is due to the smaller capacity in \methodrepresentation, which limits its expression ability as well as the amount of knowledge learned during pretraining.

==> arxiv submission v3/body/0444-model_size.tex <==

\paragraph{Model Size}
.
\skeleton{Results are robust against model size changes.}

==> arxiv submission v3/body/0445-mtdata.tex <==
\paragraph{Additional Machine Translation Data}

\label{subsec:ablation_mtdata}

We attribute the gain in the performance of \model mainly to pre-training on MT data. One evidence is the performance gain when using the larger OpenSubtitles as MT corpus for EN-DE in \ref{tab:main_results}.
% To further probe the influence of the additional MT data,
We also vary the amount of MT data available during pretraining on EN-DE direction. The results are plotted in Figure~\ref{fig:mtdata}. As the size of additional MT dataset increases, the MuST-C BLEU score improves significantly. This confirms the importance of massive high-quality MT data for pretraining \model. The results also help explain the relatively inferior scores on EN-PT in Table \ref{tab:main_results} which uses the OPUS100 dataset in pretraining.
% is highly different from MuST-C in the data source and sentence styles, \model may not be able to learn much useful knowledge from it. This hampers the final performance of \model.

==> arxiv submission v3/body/0446-visualization.tex <==
\paragraph{Visualization of \MethodRepresentations}

% \heng{Figure 4 is not readable in grayscale printout}

The \methodprojection is designed to only extract semantic categories of information necessary for decoding, regardless of the input modality. In this way, it can bridge the different representations of speech and text during computation and facilitate knowledge sharing between MT and ST.

To validate this motivation, we visualize them with Principal Component Analysis (PCA) in Figure \ref{fig:16memories}. Up to 100 speech-transcript paired samples are randomly chosen from the valid set. 
% We record vector values of all 16 \methodrepresentations from Chimera Mem-16 when inputs are speeches and transcripts. Then we apply PCA to project these vectors to a 2-dimensional surface. To distinguish the 16 \methodrepresentations, we label the projected vectors with 16 colors, each color related to one \methodrepresentation.
We record vector values of 16 \methodrepresentations from Chimera Mem-16 when inputs are speeches or transcripts, and apply 2-dimensional PCA. The 16 \methodrepresentations are distinguished by 16 colors.
Every ``$\cdot$'' corresponds to a \methodrepresentation from speech, and each ``+'' is a \methodrepresentation from the text. It is clear that the \methodrepresentations are highly clustered, everyone of which learns a particular region. Speech and text representations are also projected close within the same region, proving the model's ability to ignore representation differences and bridge the modality gap.

To take a closer view of the structure of each \methodrepresentation subspace, we randomly choose one \methodrepresentation and apply PCA to its corresponding cluster. The results are visualized in Figure \ref{fig:visualization}.
These samples come from 50 speech-transcript pairs.
Each pair of speech (``$\cdot$'') and transcript (``+'') share the same color and are linked through dashed lines.
% We additionally circle out some of the speech-transcript pairs and annotate them with the corresponding transcript texts.

% It is interesting to observe that the visualized \method has two nice properties. 
Two interesting properties could be observed.
First, paired speech and transcript inputs are again close to each other, even though they are coming from different modalities.
% In fact, some of the pairs almost overlap with each other.
% This demonstrates that the learned \methodrepresentation is indeed semantically informative in essence and modality-agnostic.
Second, the visualized representations are organized according to their semantic or syntactic patterns. We recognize several clusters in the figure, and annotate their transcripts with different fonts. The three annotations at the upper-right corner (Italic font) are all questions; those at the upper-left corner (wavy underlined font) all follow a simple future tense; at the bottom-left corner of the figure (underlined font) is another cluster of sentences of copular verbs. This proves that the \method that \model has learned is well-structured, and thus validates our model design.



\paragraph{Visualization of Inter-Modal Attention Alignment}

\cameraready{
"Attention" is the internal mechanism of Transformer based modules. In the design of \model, attention is used for extracting $M$ key semantic categories of features from input. To investigate whether these extracted features is indeed semantic, we further visualized the similarity between attention on paired audio and text in Fig \ref{fig:attention}. Here the colors, which distinguish different memories attending to inputs, is clustered on sequence and distributed close to the diagonal, demonstrating an alignment between matching tokens in two modalities. Here we also observe four beaming columns, where the full stop mark in text aligns with pauses in audio. This is an indication of semantic rather than positional essence of the memories.
}

==> arxiv submission v3/body/050analysis.tex <==
\section{Results and Analysis}
\label{sec:results}

\skeleton{How we could interpret the results presented in \ref{sec:exps}}


% \heng{you should provide more qualitative analysis with examples, and analyze the remaining errors and point out potential solutions.}

==> arxiv submission v3/body/060conclusion.tex <==


In this paper, we propose \model, a model capable of learning a \modelfullname for bridging the gap between speech and text representations. Being able to leverage a large amount of external Machine Translation data, \model achieves new state-of-the-art performance on the MuST-C dataset on all 8 languages. Additional experiment results also demonstrate its ability to learn a well-structured \method as well as effectively share learned knowledge across MT and ST, and validate our design of auxiliary tasks.

In the future, we will focus on deriving a better task to tightly align speech and text representations. Also, the workflows of MT and ST are only partially shared in \model, which still requires the model to adapt to ST when switching to the fine-tuning stage. So it remains a challenge to better couple their computation graphs in future designs.

==> arxiv submission v3/defs.tex <==

\newcommand{\xx}{\mathbf{x}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\zz}{\mathbf{z}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\hh}{\mathbf{h}}


\newcommand{\skeleton}[1]{{\color{gray} \textbf{Skeleton:} #1}}
\newcommand{\lei}[1]{{\color{blue} \textbf{Lei:} #1}}
\newcommand{\mingxuan}[1]{{\color{olive} \textbf{Mingxuan:} #1}}
\newcommand{\hanchi}[1]{{\color{cyan} \textbf{Chi:} #1}}
\newcommand{\chengqi}[1]{{\color{magenta} \textbf{Chengqi:} #1}}
\newcommand{\rong}[1]{{\color{orange} \textbf{Rong:} #1}}
\newcommand{\qianqian}[1]{{\color{teal} \textbf{Qianqian:} #1}}
\newcommand{\liming}[1]{{\color{pink} \textbf{Liming:} #1}}
\newcommand{\guest}[2]{{\color{purple} \textbf{Guest #1:} #2}}

% \newcommand{\cameraready}[1]{{\color{red} #1}}
\newcommand{\cameraready}[1]{{ #1}}

==> arxiv submission v3/fig/16memories.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{fig/16memories_v1.pdf}

\caption{2-dimensional PCA projection of the \methodrepresentations in Mem16 \model across different samples. Each colored cluster (circled out) represents a \methodrepresentation element,. A ``$\cdot$'' corresponds to a speech \methodrepresentation , and a ``+'' marks a text one.}

\label{fig:16memories}
\end{figure}

==> arxiv submission v3/fig/attention_map.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{fig/attention_map_white.pdf}
\vspace{-2em}
\caption{
\cameraready{
Visualization of the final-layer attention of $M=16$ memories on inputs, and their alignment between each other. A pair of audio and its transcript is fed to \model Mem-16. The area of each dot is linear to dot product between two attention vectors. The color is a linear interpolation of $M$ indicative colors as in Fig \ref{fig:16memories}, with mixing weights linear to the Hadamard product of attention vectors. (Best viewed in color)
}
}

\label{fig:attention}
\end{figure*}

==> arxiv submission v3/fig/contrastive.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{fig/contrastive_v3.pdf}
\caption{Besides MT and ST translation loss, we adopt a bi-modal contrastive loss to help aligning the \methodrepresentations from text and speech. In short, among \methodrepresentation elements from both sides of paired speech and transcript, the contrastive loss maximizes the cosine similarity between the same \methodrepresentation element.}
\label{fig:contrastive}
\end{figure}

==> arxiv submission v3/fig/method.tex <==

\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{fig/method_v3.pdf}

\caption{An overview of the proposed \model. The Encoder Module contains Word embedding for text input, and Wav2vec2 sub-module for speech input. The \methodprojection Module uses its \methodembedding to produce \methodrepresentation with fixed-size representation from contextual features. The Decoder Module decodes translation from the \methodrepresentation.}

\label{fig:method}
\end{figure*}


==> arxiv submission v3/fig/mt_size.tex <==
\begin{figure}[t!]
\centering

\subfloat[a][Chimera Mem-16 on WMT14]{
\includegraphics[width=0.45\textwidth]{fig/mt-size.pdf}
}

\subfloat[c][Chimera w/ and w/o OpenSubtitles]{
\begin{tabular}{cc|cc}
\toprule

Corpora & Size & MT & ST \\ \midrule
WMT14 & 4M & 32.1 & 26.3 \\
WMT14 + OpenSubtitles & 26M & 32.9 & 27.1 \\
\bottomrule

\end{tabular}
}

\caption{
\cameraready{
Curve of MuST-C EN-DE tst-COMMON BLEU scores on \model against the amount of MT data used during pretraining. (a) shows \model Mem-16's performance on WMT14. Blue triangles are the speech translation BLEU scores, and green squares are transcript-translation BLEU scores after MT pretraining. (b) shows how \model ($M=64$) behaves with or without OpenSubtitles data.
}
}
\label{fig:mtdata}
\end{figure}

==> arxiv submission v3/fig/visualization.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.7\textwidth]{fig/semantics_v4.pdf}

\caption{A visualization of one particular \methodrepresentation in Mem-16 \model no different samples and modalities. ``$\cdot$'' marks speech representations, and ``+'' marks text representations. Marks of the same color come from the same speech-transcript pair and are linked with dashed lines. Some of speech-transcript pairs are circled together and annotated with their transcripts. Three fonts distinguish three groups of transcripts of similar patterns.}

\label{fig:visualization}
\end{figure*}

==> arxiv submission v3/legacy/000abstract.tex <==
There are common semantics shared across text and images. 
Given a sentence in a source language, whether depicting the visual scene helps translation into a target language?
Existing multimodal neural machine translation methods (MNMT) require triplets of bilingual sentence - image for training and tuples of source sentence - image for inference.
In this paper, we propose \method, a novel machine translation method via visual imagination. 
\method first learns to generate visual representation from the source sentence, and then utilize both source sentence and the ``imagined representation‘’ to produce a target translation.
Unlike previous methods, it only needs the source sentence at the inference time. 
Experiments demonstrate that \method benefits from visual imagination and significantly outperforms the text-only neural machine translation baselines. 
Further analysis reveals that the imagination process in \method  help fill in missing information when performing the degradation strategy. 



% There are thousands of languages on earth, many with distinct characters.
% In contrast, visual illustration can be perceived among peoples. 
% Existing multimodal neural machine translation (MNMT) methods achieve knowledge transfer by enforcing one encoder to learn shared representation across textual and visual modalities. 
% However, these methods rely on well-aligned bilingual sentence - image triplets as the training data and the source sentence - image tuples as the inference input, which are limited in practice. 
% In this paper, we hypothesize that visual imagination via synthesizing visual representation from source text could help the neural model map two languages with different symbols, thus helps the translation task. Our proposed end-to-end imagination-based machine translation model (\method) first learns to generate semantic-consistent visual representation from source sentence, and then generate target sentence based on both text representation and imagined visual representation. Experiments demonstrate that our translation model benefits from visual imagination and significantly outperforms the text-only neural machine translation (NMT) baseline. We also conduct analyzing experiments, and the results show that imagination can help fill in missing information when performing the degradation strategy. 

==> arxiv submission v3/legacy/010intro.tex <==
Visual foundation has been introduced in a novel multimodal Neural Machine Translation (MNMT) task~\citep{specia2016shared,elliott2017findings,barrault2018findings}, which uses bilingual (or multilingual) parallel corpora annotated by images describing sentences' contents (see Figure \ref{fig1}(a)). The superiority of MNMT lies in its ability to use visual information to improve the quality of translation, but its effectiveness largely depends on the availability of data sets, especially the quantity and quality of annotated images. In addition, because the cost of manual image annotation is relatively high, at this stage, MNMT is mostly applied on a small and specific dataset, Multi30K~\cite{elliott2016multi30k}, and is not suitable for large-scale text-only Neural Machine Translation (NMT)~\cite{bahdanau2014neural,vaswani2017attention}. Such limitations hinder the applicability of visual information in NMT.

\begin{figure}[!t]
\centering
\subfigure[Multi-modal NMT]
{
\centering
\includegraphics[width=0.7\columnwidth]{fig/MNMT.pdf}
}
\subfigure[\method]
{
\centering
\includegraphics[width=0.95\columnwidth]{fig/ImagiNMT.pdf}
}
\caption{The problem setup of our proposed \method is different from existing multi-modal NMT. A multi-modal NMT model takes both text and paired image as the input, while \method takes only sentence in the source language as the usual MT task. \method synthesizes an image and utilize the internal visual representation to assist translation. }
\label{fig1}
\end{figure}

%To solve the aforementioned bottlenecks, some proposed to build a lookup table from image dataset, and then use the search-based method to retrieve pictures that match the keywords in the source language. However, the semantic meaning of the entire sentence isn't captured in their model, and the lookup table is built from Multi30K, so the coverage of the pictures is relatively narrow, and the retrieved pictures is not the reconstruction of the entire sentence, containing a lot of irrelevant noise.

To address the bottlenecks mentioned above, \citet{zhang2019neural} propose to build a lookup table from an image dataset and then using the search-based method to retrieve pictures that match the source language keywords. 
However, the lookup table is built from Multi30K, which leads to a relatively limited coverage of the pictures, and potentially  introduce much irrelevant noise. 
It does not always find the exact image corresponding to the text or the image may not even exist in the database. 
\citet{elliott2017imagination} present a multitask learning framework to ground visual representation to a shared space. 
Their architecture called "imagination" shares an encoder between a primary NMT task and an auxiliary task of ranking the visual features for image retrieval. 
However, neither the image is explicitly generated, nor the visual feature is directly leveraged by the translation decoder, the model simply learns the visual grounded shared encoder. Based on other researchers' earlier exploration, we hypothesize that the potential of vision in conventional text-only NMT has not been fully discovered. Instead, we want to explicitly imagine a "vague figure" (see Figure \ref{fig1}(b)) to guide the translation, since \emph{A picture is worth a thousand words}, and imagining the picture of a sentence is the instinctive reaction of a human being who is learning bilingualism.

In this paper, we propose a novel end-to-end machine translation model that is embedded in visual semantics with generative imagination (\method) (see Figure \ref{fig1}(b)). Given a source language sentence, \method first encodes it and transforms the word representations into visual features through an attentive generator, which can effectively capture the semantics of both global and local levels, and the generated visual representations can be considered as semantic-equivalent reconstructions of sentences. A simple yet effective integration module is designed to aggregate the textual and visual modalities. In the final stage, the model learns to generate the target language sentence based on the joint features. To train the model in an end-to-end fashion, we apply a visual realism adversarial loss and a text-image pair-aware adversarial loss, as well as text-semantic reconstruction loss and target language translation loss based on cross-entropy. 

%Furthermore, we also incorporate a triplet ranking loss to make the generated visual feature close to the matched text in the latent visual semantic space.

In contrast with most prior MNMT work, our proposed \method model does not require images as input during the inference time but can leverage visual information through imagination, making it an appealing method in low-resource scenario. Moreover, \method is also flexible, accepting external parallel text data or non-parallel image captioning data. We evaluate our Imagination modal on the Multi30K dataset. The experiment results show that our proposed method significantly outperforms the text-only NMT baseline. The analysis demonstrates that imagination help the model complete the missing information in the sentence when we perform degradation masking, and we also see improvements in translation quality by pre-training the model with an external non-parallel image captioning dataset.

To summarize, the paper has the following contributions: 
\begin{enumerate}
    \item We propose generative imagination, a new setup for machine translation assisted by synthesized visual representation, without annotated images as input;
    \item We propose the \method method, which shows advantages over the conventional MNMT model and gains significant improvements over the text-only NMT baseline;
    \item We conduct experiments to verify and analyze how imagination helps the translation.
\end{enumerate}

==> arxiv submission v3/legacy/020related.tex <==
%Using additional knowledge to construct fine-grained representations is an important issue in language modeling. However, 
\textbf{MNMT}   As a language shared by people worldwide, visual modality may help machines have a more comprehensive perception of the real world. Multimodal neural machine translation (MNMT) is a novel machine translation task proposed by the machine translation community, which aims to design multimodal translation frameworks using context from the additional visual modality \cite{specia2016shared}. The shared task release the dataset Multi30K~\cite{elliott2016multi30k}, which is an extended German version of Flickr30K~\cite{young2014image}, then expanded to French and Czech~\cite{elliott2017findings,barrault2018findings}. In the three versions of tasks, scholars have proposed many multimodal machine translation models and methods. \citet{huang2016attention}  encodes word sequences with regional visual objects, while \citet{calixto2017incorporating} study the effects of incorporating global visual features to initialize the encoder/decoder hidden states of RNN. \citet{caglayan2017lium} models the image-text interaction by leveraging element-wise multiplication. \citet{elliott2017imagination} proposed a multitask learning framework to ground visual representation to a shared space and learn with the auxiliary triplet alignment task. The common practice is to use convolutional neural networks to extract visual information and then using attention mechanisms to extract visual contexts~\cite{caglayan2016multimodal,calixto2016dcu,libovicky2017attention}. \citet{ive2019distilling}  propose a translate-and-refine approach using two-stage decoder. \citet{calixto2018latent} put forward a latent variable model to capture the multimodal interactions between visual and textual features. \citet{caglayan2019probing} show that visual content is more critical when the textual content is limited or uncertain in MMT. Recently, \citet{yao2020multimodal} propose multi-modal self-attention in Transformer to avoid encoding irrelevant information in images, and \citet{yin2020novel} propose a graph-based multimodal fusion encoder to capture various relationships.

%(2) Cross-modal interaction using spatially agnostic global information (\cite{calixto2017incorporating}; \cite{ma2017osu}; \cite{caglayan2017lium}); (3) Regional feature integration from the target detection network (\cite{huang2016attention}; \cite{gronroos2018memad}).

\textbf{Text-to-image synthesis}   Traditional Text-to-image (T2I) synthesis mainly uses keywords to search for small image regions, and finally optimizes the entire layout~\cite{zhu2007text}. After generative adversarial networks (GANs)~\cite{goodfellow2014generative} were proposed, scholars have presented a variety of GAN-based T2I models. \citet{reed2016generative} propose DC-GAN and design a direct and straightforward network and a training strategy for T2I generation. \citet{zhang2017stackgan} propose stackGAN, which contains multiple cascaded generators and discriminators, and the higher stage generates better quality pictures. In previous work, scholars only considered global semantics. \citet{xu2018attngan} proposed AttnGAN to apply the attention mechanism to capture fine-grained word-level information. MirrorGAN~\cite{qiao2019mirrorgan} employs a mirror structure, which reversely learns from the inverse task of T2I to further validate whether generated images are consistent with the input texts. The inverse task is also known as image captioning.

==> arxiv submission v3/legacy/030method.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{fig/model.pdf} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Overview of the framework of the proposed \method. $F_{0}$ and $F_{1}$ are text-to-image converters, comprising of perceptron, residual, and unsampling blocks. L $\times$ represents L identical layers. Noting that we only need to obtain the generated visual feature to guide the translation, up-sampling this feature to image is redundant.}
\label{fig2}
\end{figure*}

As shown in Figure\ref{fig2}, \method embodies the encoder-decoder structure for end-to-end machine translation. Between the encoder and the decoder, there is an imagination step to generate semantic-equivalent visual representation. Technically, our model is composed of following modules: source text encoder, generative imagination network, image captioning, and decoder for translation. We will elaborate on each of them in the rest of this section.

\subsection{Source text encoder}

\citet{vaswani2017attention} propose the state-of-art Transformer-based machine translation framework, which can be written as follows:

\begin{equation}
    \overline{\textbf{H}}^{l}=\textit{LN}(\textit{Att}^{l}(\textbf{Q}^{l-1},\textbf{K}^{l-1},\textbf{V}^{l-1})+\textbf{H}^{l-1}),
\end{equation}

\begin{equation}
    \textbf{H}^{l}=\textit{LN}(\textit{FFN}^{l}(\overline{H}^{l})+\overline{H}^{l}),
\end{equation}

Where $\textit{Att}^{l}$, $\textit{LN}$, and $\textit{FFN}^{l}$ are the self-attention module, layer normalization, and the feed-forward network for the $l$-th identical layer respectively. The core of the Transformer is the multi-head self-attention, in each attention head, we have:

\begin{equation}
    z_{i}=\sum_{j=1}^{n}\alpha_{ij}(x_{j}W^{V}),
\end{equation}

\begin{equation}
    \alpha_{ij}=softmax(\frac{(x_{i}W^{Q})(x_{j}W^{K})^\top }{\sqrt{d}}),
\end{equation}

$W^{V},W^{Q},W^{K}$ are layer-specific trainable parameter matrices. For the output of final stacked layer, we use $w=\{w_{0},w_{1},...,w_{L-1} \}$, $w\in\mathbb{R}^{d\times L}$ to represent the source word embedding, $L$ is the length of the source sentence. Besides, we add a special token to each source language sentence to obtain the sentence representation $s \in \mathbb{R}^{d}$.

\subsection{Generative imagination network}

Generative Adversarial Network~\cite{goodfellow2014generative} has been applied to synthesis images similar to ground truth~\cite{zhang2017stackgan,xu2018attngan,qiao2019mirrorgan}. We follow the common practice of using the conditioning augmentation~\cite{zhang2017stackgan} to enhance robustness to small perturbations along the conditioning text manifold. $F^{ca}$ represents the conditioning augmentation function, and $s^{ca}$ represents the enhanced sentence representation.

\begin{equation}
    s^{ca}=F^{ca}(s),
\end{equation}

$\{F_{0}, F_{1}\}$ are two visual feature converters, including perceptron, residual and upsampling layers. Furthermore, we define $\{f_{0}, f_{1}\}$ are the visual features after two transformations. For detailed layer structure and block design, please refer to ~\cite{xu2018attngan}.

\begin{equation}
    f_{0}=F_{0}(z,s^{ca}),
\end{equation}

\begin{equation}
    f_{1}=F_{1}(f_{0},F^{attn}(f_{0},s^{ca})),
\end{equation}

$z$ is the noise vector, sampled from the standard normal distribution, and it will be concatenated with $s^{ca}$. $f_{0}\in \mathbb{R}^{M_{0}\times N_{0}}$. Each column of $f_{i}$ is a feature vector of a sub-region of the image, which can also be treat as a pseudo-token. To generate fine-grained details at different subregions of the image by paying attention to the relevant words in the source language, we use image vector in each sub-region to query word vectors by leveraging attention strategy. $F^{attn}$ is an attentive function to obtain word-context feature, then we have:

\begin{small}
\begin{equation}
    F^{attn}(f_{0},s^{ca})=\sum _{l=0}^{L-1} (U_{0}w_{l})(softmax(f_{0}^{T}(U_{0}w_{l})))^\top 
\end{equation}
\end{small}


Word feature $w_{l}$ is firstly converted into the common semantic space of the image feature, $U_{0}$ is a perceptron layer. Then it will be multiplied with visual feature $f_{0}$ to acquire the attention score. $f_{1}$ is the output of the imagination network, capturing multiple levels (word level and sentence level) of semantic meaning. It will be utilized directly for target language generation, and it will also be passed to the discriminator for adversarial training.

\subsection{Image captioning}

Image captioning (I2T) can be regarded as the inverse problem of text-to-image generation, generating the given image's description. If an imagined image is semantic equivalent to the source sentence, then its description should be almost identical to the given text. Thus we leverage the image captioning to translate the imagined visual representation back to the source language\cite{qiao2019mirrorgan}, and this symmetric structure can make the imagined visual feature act like a mirror, effectively enhancing the semantic consistency of the imagined visual feature and precisely reflect the underlying semantics. Following \citet{qiao2019mirrorgan}, we utilize the widely used encoder-decoder image captioning framework\cite{vinyals2015show}, and fix the parameter of the pre-trained image captioning framework when end-to-end training other modules in \method.

\begin{equation}
    p_{t}=Decoder(h_{t-1}),t=0,1,...,L-1.
\end{equation}

\begin{equation}
    \mathcal{L}_{I2T} = -\sum_{t=0}^{L-1} \log p_{t}(T_{t}),
    \label{equation10}
\end{equation}

$p_{t}$ is the predicted probability distribution over the words at $t_{0}$-th decoding step, and $T_{t}$ is the $T_{t}$-th entry of the probability vector.

%\subsection{Aligning the VSE space}

%In this section, we align a shared visual-semantic embedding (VSE) space to find a good distributed representation that can capture the semantic meaning across two modalities. Drawing the generated visual representation and the corresponding sentence closer contributes to better semantic alignment in the language latent space, and it can also encourage the imagination network to validate the semantic consistency further.

%Specifically, we leverage the contrastive triplet loss in cross-modal retrieval to encourage the textual-visual alignment in the VSE space~\cite{kiros2014unifying,lee2018stacked}. Furthermore, we utilize fine-grained and bidirectional (textual-to-visual, visual-to-textual) attention mechanisms to learn to value the imagined visual representation with close semantic relatedness to the source sentence. We denote $h^{f}$ to represent object-level visual feature, and $h^{w}$ to represent the token-level textual feature. The visually-attend textual representation $h^{fw}$ is the weighted combination of $h^{w}$. Similarly, $h^{wf}$ represents textually-attend visual representation. For visual-aware attention, we have:

%\begin{equation}
%    h_{j}^{fw} = \sum_{i=0}^{L-1}\alpha_{ij}h_{i}^{w},
%\end{equation}

%\begin{equation}
%    \alpha_{ij}=softmax_{i}(cos(h_{i}^{w},h_{j}^{f})),
%\end{equation}

%Where $j = 0, ..., M-1$. $L$ is the sentence length, and $M$ is the visual feature maps. Then we get:

%\begin{equation}
%\begin{split}
%    S(f,w)=\frac{1}{2M}\sum_{j=0}^{M-1}cos(h_{j}^{fw},h_{j}^{f}) \\
%    +\frac{1}{2L}\sum_{i=0}^{L-1}cos(h_{i}^{wf},h_{i}^{w}) &
%\end{split}
%\end{equation}

%\begin{equation}
%\begin{split}
%    \mathcal{L}_{c}(f,w) = \max_{\Tilde{f}}[\gamma-S(f,w)+S(\Tilde{f},w)]_{+} \\ + \max_{\Tilde{w}}[\gamma-S(f,w)+S(f,\Tilde{w})]_{+} &
%\end{split}
%\end{equation}

%$S(f,w)$ is the cosine similarity between a sentence and an image, $\mathcal{L}_{c}(f,w)$ is the contrastive triplet loss. $\Tilde{f}$ and $\Tilde{w}$ are the contrastive non-paired example with respect to the selected source text and the selected imagined visual representation. $[]_{+}$ is the hinge loss function. When the loss decreases, the distance between a paired image and sentence will drop while the distance between an unpaired image and sentence increases. 

\subsection{Multimodal aggregation}

After obtaining the imagined visual representation, we aggregate two modalities for the translation decoder. Although the vision carries richer information, it also contains irrelevant noise. Comparing to encoding and integrating visual feature directly, a more elegant method is to induce the hidden representation under the guide of image-aware attention and graph perspective of transformer~\cite{yao2020multimodal}, since each local spatial regions of the image can also be considered as pseudo-tokens, which can be added to the source fully-connected graph. In the multimodal self-attention layer, we add the spatial feature of the generated feature map in the source sentence, getting $\Tilde{x}\in\mathbb{R}^{(L+M)\times d}$, then perform image-aware attention, we have:

\begin{equation}
    c_{i}=\sum_{j=0}^{L-1}\Tilde{\alpha}_{ij}(w_{j}W^{V})
\end{equation}

\begin{equation}
    \Tilde{\alpha}_{ij}=softmax(\frac{(\Tilde{x}_{i}W^{Q})(w_{j}W^{K})^\top }{\sqrt{d}})
\end{equation}

\subsection{Objective function}

\begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{fig/loss1.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Training objective. The discriminator takes source language sentences, generated images, and real images as input, then computes two adversarial loss: realism loss and text-image paired loss. $\mathcal{L}_{I2T}$ is designed to guarantee the semantic consistency, and $\mathcal{L}_{trans}$ is the core loss function to translate integrated embedding to the target language.}
\label{fig3}
\end{figure}

During the translation phase, similar to equation\ref{equation10}, we have:

\begin{equation}
    \mathcal{L}_{trans} = -\sum_{t} \log p_{t}(T_{t})
\end{equation}

To train the whole network end-to-end, we leverage adversarial training to alternatively train the generator and the discriminator. Especially, as shown in Figure\ref{fig3}, the discriminator take the imagined visual representation, source language sentence, and the real image as input, and we employ two adversarial losses: a visual realism adversarial loss, and a text-image pair-aware adversarial loss computed by the discriminator~\cite{zhang2017stackgan,xu2018attngan,qiao2019mirrorgan}. 

\begin{equation}
\begin{split}
        \mathcal{L}_{G_{0}}=-\frac{1}{2}\mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(D(I_{i})]\\ -\frac{1}{2}\mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(D(I_{i},s)]&
\end{split}
\end{equation}

The first term is to distinguish real and fake, ensuring that the generator generates visually realistic images. The second term is to guarantee the semantic consistency between the input text and the generated image. The final objective function of the generator is defined as:

\begin{equation}
    \mathcal{L}_{G}=\mathcal{L}_{G_{0}}+\lambda_{1}\mathcal{L}_{I2T}+ \lambda_{2}\mathcal{L}_{trans}
\end{equation}

Accordingly, the discriminator $D$ is trained by minimizing the following loss:

\begin{equation}
\begin{split}
    L_{D} =-\frac{1}{2} \mathbb{E}_{I_{i}^{GT}\sim p_{I_{i}^{G}}}[\log(D(I_{i}^{GT})]\\
    -\frac{1}{2} \mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(1-(I_{i})] \\
    -\frac{1}{2} \mathbb{E}_{I_{i}^{GT}\sim p_{I_{i}^{G}}}[\log(D(I_{i}^{GT},s)]\\
    -\frac{1}{2} \mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(1-D(I_{i},s)]&
\end{split}
\end{equation}

==> arxiv submission v3/legacy/040experiment.tex <==
\subsection{Datasets}

\begin{table*}[ht]
\centering
\small
\linespread{1.2}
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{l|cccccc}
\hline
\multirow{3}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{En$\Rightarrow$De}}  \\
\cline{2-7}
& \multicolumn{2}{c}{\textbf{Test2016}}  
& \multicolumn{2}{c}{\textbf{Test2017}} 
& \multicolumn{2}{c}{\textbf{Ambiguous COCO}} \\
\cline{2-7}
& BLEU & METEOR & BLEU & METEOR & BLEU & METEOR \\
\hline
\hline
\multicolumn{7}{c}{\emph{Multimodal Neural Machine Translation Systems}} \\
\hline
IMG$_{D}$ ~\cite{calixto2017incorporating} & 37.3 & 55.1 & N/A & N/A & N/A & N/A \\
NMT$_{SRC+IMG}$ ~\cite{calixto2017doubly}  & 36.5 & 55.0 & N/A & N/A & N/A & N/A  \\
trg-mul ~\cite{caglayan2017lium} & 37.8 & \textbf{57.7} & 30.7 & 52.2 & 27.1 & 47.2 \\
VAG-NMT ~\cite{zhou2018visual} & N/A & N/A & 31.6 & 52.2 & 28.3 & 48.0 \\
Transformer+Att ~\cite{ive2019distilling} & 38.0 & 55.6 & N/A & N/A & N/A & N/A \\
Multimodal transformer ~\cite{yao2020multimodal} & 38.7 & 55.7 & N/A & N/A & N/A & N/A \\
\method + ground truth & 38.6 & 55.7 & 32.4 & 52.5 & 28.8 & 48.9 \\
\hline
\multicolumn{7}{c}{\emph{Text-only Neural Machine Translation Systems}} \\
\hline
Transformer baseline ~\cite{vaswani2017attention} & 37.6 & 55.3 & 31.7 & 52.1 & 27.9 & 47.8 \\
Multitask ~\cite{elliott2017imagination} & 36.8 & 55.8 & 30.2 & 51.2 & N/A & N/A \\
VMMT$_{F}$~\cite{calixto2018latent} & 37.6 & 56.0 & N/A & N/A & N/A & N/A \\
Lookup table ~\cite{zhang2019neural} & 36.9 & N/A & 28.6 & N/A & N/A & N/A \\
\method & 38.5 & 55.7 & 32.1 & 52.4 & 28.7 & 48.8 \\
\hline
\end{tabular}}
\caption{Main result from the Test2016, Test2017, and Ambiguous COCO for the En$\Rightarrow$De MNMT task. The first category collects the existing MNMT systems, which take both source sentences and paired images as input. The second category illustrates the systems that do not require images as input. Since our method falls into the second group, our baseline are the text-only transformer~\cite{vaswani2017attention} and the aforementioned works~\cite{zhang2019neural,elliott2017imagination}.}
\label{Table_En2DeMainResults}
\end{table*}

We evaluate our proposed \method model on two datasets, Multi30K~\cite{elliott2016multi30k} and Ambiguous COCO~\cite{elliott2017findings}. To show its ability to train with external out-of-domain datasets, we adopt MS COCO~\cite{lin2014microsoft} in the next analyzing section.

Multi30K is the largest existing human-labeled collection for MNMT, containing $31K$ images and consisting of two multilingual expansions of the original Flickr30K\cite{young2014image} dataset. The first expansion has five English descriptions and five German descriptions, and they are independent of each other. The second expansion has one of its English description manually translated to German by a professional translator, then expanded to French and Czech in the following shared task~\cite{elliott2017findings,barrault2018findings}. We only apply the second expansion in our experiments, which has $29,000$ instances for training, $1,014$ for development, and $1,000$ for evaluation. We present our results on English-German (En-De) Test2016 and Test2017.

Ambiguous COCO is a small evaluation dataset collected in the WMT2017 multimodal machine translation challenge~\cite{elliott2017findings}, which collected and translated a set of image descriptions that potentially contain ambiguous verbs. It contains $461$ images from the MS COCO\cite{lin2014microsoft} for $56$ ambiguous vers in total. 

MS COCO is the widely used non-parallel text-image paired dataset in T2I and I2T generation. It contains $82,783$ training images and $40,504$ validation images with $91$ different object types, and each image has 5 English descriptions.

\subsection{Settings}

Our baseline is the conventional text-only Transformer~\cite{vaswani2017attention}. Specifically, each encoder-decoder has a 6-layer stacked Transformer network, eight heads, 512 hidden units, and the inner feed-forward layer filter size is set to 2048. The dropout is set to $p=0.1$, and we use Adam optimizer~\cite{kingma2014adam} to tune the parameter. The learning rate increases linearly for the warmup strategy with $8,000$ steps and decreases with the step number's inverse square root. We train the model up to $10,000$ steps, the early-stop strategy is adopted. We use the same setting as \citet{vaswani2017attention}. We use the metrics BLEU~\cite{papineni-etal-2002-bleu} and METEOR~\cite{denkowski-lavie-2014-meteor}to evaluate the translation quality.

For the imagination network, the noise vector's dimension is $100$, and the generated visual feature is $128\times128$. The upsampling and residual block in visual feature transformers consist of $3\times3$ stride 1 convolution, batch normalization, and ReLU activation. The training is early-stopped if the dev set BLEU score do not improve for $10$ epochs, since the translation is the core task. The batch size is $64$, and the learning rate is initialized to be $2e^{-4}$ and decayed to half of its previous value every $100$ epochs. A similar learning schedule is adopted in \citet{zhang2017stackgan}. The margin size $\gamma$ is set to $0.1$, the balance weight $\lambda_{1}=20$, $\lambda_{2}=40$. 

\subsection{Results}

Table \ref{Table_En2DeMainResults} illustrates the results for the Test2016, Test2017, and the Ambiguous COCO MNMT tasks. Our text-only Transformer baseline~\cite{vaswani2017attention} has similar results compared to most prior MNMT works, which is consistent with the previous findings~\cite{caglayan2019probing}, that is, textual modality is good enough to translate for Multi30K dataset. This finding helps to explain that it is already tricky for a MNMT model to ground visual modality even with the presence of annotated images. However, Our \method gains improvements over the text-only Transformer baseline on three evaluation datasets, demonstrating that our model can effectively embed the visual semantics during the training time and guide the translation through imagination with the absence of annotated images during the inference time. We assume much of the performance improvement is due to \method's strong ability to capture the interaction between text and image, generate semantic-consistent visual representations, and incorporate information from visual modality properly. 

We also observe that our approach surpasses the results of most MNMT systems by a noticeable margin in terms of BLEU score and METEOR score on three evaluation dataset. Our \method is also competitive with \method + ground truth, which is our translation decoder taking ground truth visual representations instead of imagined ones. This proves imaginative ability of \method.

For Ambiguous COCO, which was purposely curated such that verbs have ambiguous meaning, demands more visual contribution for guiding the translation and selecting correct words. Our \method benefits from visual imagination and substantially outperforms previous works on ambiguous COCO.

\subsection{Ablation studies}

\begin{table}[ht]
\centering
\begin{tabular}{l|cc}
\hline
 Evaluation metric             & BLEU   & METEOR     \\ \hline
 ImagiT, $\lambda_{1}=0$ & 37.9 & 55.3 \\ \hline
  ImagiT, $\lambda_{1}=5$ & 38.2 & 55.5 \\ \hline
   ImagiT, $\lambda_{1}=10$ & 38.4 & 55.7 \\ \hline
    ImagiT, $\lambda_{1}=20$ & 38.5 & 55.7 \\ \hline
     ImagiT, $\lambda_{1}=40$ & 38.3 & 55.6 \\ \hline
\end{tabular}
\caption{Ablation studies of ImagiT with different weight settings}
\label{table2}
\end{table}

The hyper-parameter $\lambda_{1}$ is important. When $\lambda_{1}=0$, there is no image captioning component, the BLEU score drops from 38.6 to 37.9, while this variant still outperforms the Transformer baseline. This indicates the effectiveness of image captioning module, since it will potentially prevent visual-textual mismatching, thus helps generator achieve better performance. When $\lambda_{1}$ increases from $5$ to $20$, the BLEU and METEOR increase accordingly. Whereas $\lambda_{1}$ is set to equal to $\lambda_{2}$ ($40$), the BLEU score falls to 38.4. That's reasonable because $\lambda_{2}\mathcal{L}_{trans}$ is the main task of the whole model.

==> arxiv submission v3/legacy/050analyse.tex <==
\subsection{Can \method generate visual grounded representations?}

Since the proposed model does not require images as input, one may ask how it uses visual information and where the information comes? We claim that \method has already been embedded with visual semantics during the training phase, and in this section, we validate that \method is able to generate visual grounded representation by performing the image retrieval task.

For each source sentence, we generate the intermediate visual representation. Furthermore, we query the ground truth image features for each generated representation to find the closest image vectors around it based on the cosine similarity. Then we can measure the $R@K$ score, which computes the recall rate of the matched image in the top K nearest neighborhoods.

\begin{table}[h]
\centering
\begin{tabular}{l|ccc}
\hline
              & $R@1$     & $R@5$ &  $R@10$   \\ \hline
\method on Multi30K & 64.7  & 88.7 & 94.2 \\ \hline
\method on MS COCO & 64.3  &  89.5   & 94.7 \\
\hline
\end{tabular}
\caption{Image retrieval task. We evaluate on Multi30K and MS COCO.}
\label{retrieval}
\end{table}

Some previous studies on VSE perform sentence-to-image retrieval and image-to-sentence retrieval, but their results can not be directly compared with ours, since we are performing image-to-image retrieval in practical. However, from Table \ref{retrieval}, especially for $R@10$, the results demonstrate that our generated representation has excellent quality of shared semantics and have been grounded with visual semantic-consistency. 

\subsection{How does the imagination help the translation?}

Although we have validated the effectiveness of \method on three widely used MNMT evaluation datasets. A natural question to ask is that how does the imagination guide the translation, and to which extent? When human beings confronting with complicate sentences and obscure words, we often resort to mind-picturing and mental visualization to assist us to auto-complete and fill the whole imagination. Thus we hypothesis that imagination could help recover and retrieve the missing and implicate textual information.

Inspired by \citet{ive2019distilling,caglayan2019probing}, we apply degradation strategy to the input source language, and feed to the trained Transformer baseline, MNMT baseline, and \method respectively, to validate if our proposed approach could recover the missing information and obtain better performance. And we conduct the analysing experiments on En-De Test2016 evaluation set.

\textbf{Color deprivation} is to mask the source tokens that refers to colors, and replace them with a special token [M]. Under this circumstance, text-only NMT model have to rely on source-side contextual information and biases, while for MNMT model, it can directly utilize the paired color-related information-rich images. But for \method, the model will turn to imagination and visualization.

\begin{table}[!h]
\centering
\begin{tabular}{l|cc}
\hline
 Model             & $S$     & $\overline{S}$    \\ \hline
text-only Transformer & 37.6  & 36.3 \\ \hline
MNMT        & 38.2 & 37.7 \\ \hline
\method       & 38.4 & 37.9 \\
\hline
\end{tabular}
\caption{Color deprivation. $s$ represents the original source sentence, while $\overline{s}$ is the degraded sentence.}
\label{color deprivation}
\end{table}

Table ~\ref{color deprivation} demonstrates the results of color deprivation. We implement a simple transformer-based MNMT baseline model using the multimodal self-attention approach~\cite{yao2020multimodal}. Thus the illustrated three models in Table\ref{table2} can be compared directly. We can observe that the BLEU score of text-only NMT decreases 1.3, whereas MNMT and \method system only decreases 0.5. This result corroborates that our \method has a similar ability to recover color compared to MNMT, but our \method achieves the same effect through its own efforts, i.e., imagination.

\textbf{Visually depictable entity masking}. \citet{plummer2015flickr30k} extend Flickr30K with cereference chains to tag mentions of visually depictable entities. Similar to color deprivation, we randomly replace $0\%,15\%,30\%,45\%,60\%$ visually depictable entities with a special token [M].

\begin{figure}[h]
\centering
\includegraphics[width=0.95\columnwidth]{fig/analyse.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Visually depictable entity masking. From top to bottom is MNMT, \method, text-only transformer.}
\label{fig4}
\end{figure}

Figure~\ref{fig4} is the result of visually depictable entity masking. We observe a large BLEU score drop of text-only Transformer baseline with the increasing of masking proportion, while MNMT and \method are relatively smaller. This result demonstrates that our \method model can much more effectively infer and imagine missing entities compared to text-only Transformer, and have comparable capability over the MNMT model.

\subsection{Will better imagination with external data render better translation?}

Our \method model also accepts external parallel text data or non-parallel image captioning data, and we can easily modify the objective function to train with out-of-domain non-triple data. To train with text-image paired image captioning data, we can pre-train our imagination model by ignoring $\mathcal{L}_{trans}$ term. In other words, the T2I synthesis module can be solely trained with MS COCO dataset. We randomly split MS COCO in half, and use COCO$_{half}$ and COCO$_{full}$ to pre-train \method. The MS COCO is processed using the same pipeline as in \citet{zhang2017stackgan}. Furthermore, the training setting of COCO$_{half}$ and COCO$_{full}$ are the same with batch size $64$ and maximum epoch $600$. The results are:

\begin{table}[!h]
\centering
\begin{tabular}{l|cc}
\hline
              & BLEU     & METEOR    \\ \hline
\method & 38.4  & 55.7 \\ \hline
\method + COCO$_{half}$& 38.6 & 56.3 \\ \hline
\method + COCO$_{full}$& 38.7 & 56.7 \\
\hline
\end{tabular}
\caption{Translation results when using out-of-domain non-parallel image captioning data.}
\label{table3}
\end{table}

As is shown in Table\ref{table3}, our \method model pre-trained with half MS COCO gain 0.6 METEOR increase, and the improvement becomes more apparent when training with the whole MS COCO. We can contemplate that large-scale external data may further improve the performance of \method, and we have not utilized parallel text data (e.g., WMT), even image-only and monolingual text data can also be adopted to enhance the model capability, and we leave this for future work.

==> arxiv submission v3/legacy/060conclusion.tex <==
This work presents generative imagination-based machine translation model (\method), which can effectively capture the source semantics and generate semantic-consistent visual representations for imagination-guided translation. Without annotated images as input, out model gains significant improvements over text-only NMT baselines and is comparable with the SOTA MNMT model. We analyze how imagination elevates machine translation and show improvement using external image captioning data. Further work may center around introducing more parallel and non-parallel, text, and image data for different training schemes. 

==> arxiv submission v3/tables/contrastive_ablation.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{l|cc}
\toprule

 
Language & with & w/o \\
\midrule
EN-DE & 24.5 & 24.4 \\
EN-FR & 34.5 & 33.7 \\
EN-RU & 16.6 & 16.4 \\
EN-ES & 30.0 & 29.9 \\
\bottomrule

\end{tabular}
\caption{BLEU scores of \model on MuST-C tst-COMMON set with (``with'') or without (``w/o'') dual-modal contrastive trainig. Result on EN-FR shows the largest drop, proving it more necessary to align between speech and text representations for \model when MT pretraining data is larger.}
\label{tab:contrastive_ablation}

\end{table}

==> arxiv submission v3/tables/freezing_modules.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{cc|cc}
\toprule

S.S. Projection & Decoder & EN-DE & EN-FR \\ \midrule
 - & - & 25.6 & 35.0 \\
 Fixed & - & 24.3 & 34.3 \\
 - & Fixed & 24.2 & 33.4 \\
 Fixed & Fixed & 23.8 & 33.1 \\
 \bottomrule

\end{tabular}
\caption{Performance of Mem-16 \model when freezing different modules in fine-tuning. S.S. Projection is abbreviation for \methodprojection. ``Fixed'' indicates that weights in this module are not updated during fine-tuning, and ``-'' means otherwise. The results demonstrate that freezing modules indeed hampers the model's ability to adapt, but the weights pretrained on MT are already highly informative for ST.}
\label{tab:freezing}

\end{table}

==> arxiv submission v3/tables/librispeech_results.tex <==
\begin{table}[t!]
\centering
\setlength\tabcolsep{3pt}
\begin{tabular}{cccc|cc}
\toprule

\multirow{2}{*}{\textbf{Model}} &
\multicolumn{3}{c}{\textbf{External Data}} &  \multicolumn{2}{c}{\textbf{Aug-Libri}} \\
& Speech & ASR & MT & u-tok & c-detok \\
\midrule

W2V2-T $^\ast$ & \checkmark & $\times$ & $\times$ & 6.5 & 6.4 \\
TCEN $^\dagger$ & $\times$ & $\times$ & $\times$ & 17.1 & - \\
LSTM $^\ddagger$& $\times$ & \checkmark & \checkmark & 17.0 & - \\
AFS $^\circ$ & $\times$ & $\times$ & $\times$ & 18.6 & 17.2 \\
Multilingual $^\star$ & $\times$ & \checkmark & $\times$ & 17.6 & - \\
Transformer $^\bot$ & $\times$ & \checkmark &  $\times$ & 17.7 & - \\
Curiculum $^\bot$ & $\times$ & \checkmark &  $\times$ & 18.0 & - \\
COSTT $^\flat$ & $\times$ & $\times$ & \checkmark & 18.2 & - \\
LUT $^\diamondsuit$ & $\times$ & \checkmark & $\times$ & 18.3 & - \\
STAST $^\sharp$ & $\times$ & \checkmark & $\times$ & 18.7 & - \\
\midrule
% \model-abl & \checkmark & $\times$ & \checkmark & 14.3 \\
\model & \checkmark & $\times$ & \checkmark & \textbf{20.2} & \textbf{19.4} \\

\bottomrule

\end{tabular}
\caption{\cameraready{Results on LibriSpeech English-French dataset. Among baselines, 
$^\ast$ is the same W2V2-Transformer baseline as in Table \ref{tab:main_results}. 
$^\dagger$ is from ~\citet{wang2020bridging}, $^\ddagger$ from ~\citet{bahar2019using}, $^\star$ from ~\citet{inaguma2019multilingual}, two baselines under $^\bot$ from ~\citet{wang2020curriculum}, $^\flat$ from ~\citet{dong2021consecutive}, $^\diamondsuit$ from ~\citet{dong2021listen}, $^\circ$ from ~\citet{zhang2020adaptive} and $^\sharp$ from ~\citet{liu2020bridging}. ``u-tok'' represents case-insensitive tokenized BLEU, while ``c-detok'' is case-sensitive detokenized BLEU.
% \model-abl is an ablation version without auxiliary losses in pre-training.
}}

\label{tab:librispeech}
\end{table}

==> arxiv submission v3/tables/main_results.tex <==
\begin{table*}[t!]
\centering
\small
\linespread{1}

\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{lccc|cccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{External Data}} 
& \multicolumn{8}{c}{\textbf{MuST-C EN-X}}  \\
& Speech & ASR & MT 
& EN-DE & EN-FR & EN-RU & EN-ES & EN-IT & EN-RO & EN-PT & EN-NL\\
% & DE & FR & RU & ES & IT & RO & PT & NL\\

% \midrule
% \multicolumn{9}{c}{\emph{Cascaded Models}} \\
% \midrule
% Transformer ASR + CTC $\rightarrow$ Transformer MT $^\ddagger$
% & 23.7 & 33.8 & 16.4 & 28.7 & 24.0 & 22.7 & 29.0 & 27.9 \\

% \midrule

% \multicolumn{9}{c}{\emph{End-to-End Models}} \\

\midrule
FairSeq ST $^\dagger$
& $\times$ & $\times$ & $\times$ & 22.7 & 32.9 & 15.3 & 27.2 & 22.7 & 21.9 & 28.1 & 27.3 \\
Espnet ST $^\ddagger$
& $\times$ & $\times$ & $\times$ & 22.9 & 32.8 & 15.8 & 28.0 & 23.8 & 21.9 & 28.0 & 27.4 \\
AFS $^\star$
& $\times$ & $\times$ & $\times$ & 22.4 & 31.6 & 14.7 & 26.9 & 23.0 & 21.0 & 26.3 & 24.9 \\
% \model (no pretraining)
% & 19.05 & 29.24 & 12.41 & 25.12 &  &  &  &  \\
Dual-Decoder $^\diamondsuit$
& $\times$ & $\times$ & $\times$ & 23.6 & 33.5 & 15.2 & 28.1 & 24.2 & 22.9 & \textbf{30.0} & 27.6 \\
STATST $^\sharp$
& $\times$ & $\times$ & $\times$ & 23.1 & - & - & - & - & - & - & - \\
MAML $^\flat$
& $\times$ & $\times$ & \checkmark & 22.1 & 34.1 & - & - & - & - & - & - \\
Self-Training $^\circ$
& \checkmark & \checkmark & $\times$ & 25.2 & 34.5 & - & - & - & - & - & - \\

W2V2-Transformer $^\ast$
& \checkmark & $\times$ & $\times$ & 22.3 & 34.3 & 15.8 & 28.7 & 24.2 & 22.4 & 29.3 & 28.2 \\

\hline

\model Mem-16 % \hanchi{for internal only}
& \checkmark & $\times$ & \checkmark & 25.6 & 35.0 & 16.7 & 30.2 & 24.0 & 23.2 & 29.7 & 28.5 \\
% note that the EN-RO results here are not beam++ and avrg-ckpt-ed version. I lost the saved checkpoints by mistake.\

\model
& \checkmark & $\times$ & \checkmark & \textbf{27.1}$^\mathsection$ & \textbf{35.6} & \textbf{17.4} & \textbf{30.6} & \textbf{25.0} & \textbf{24.0} & \textbf{30.2} & \textbf{29.2} \\
% \model + OpenSubtitles
% & \checkmark & $^\times$ & \checkmark & \textbf{27.1} & - & - & - & - & - & - & - \\

% \model (beam size 5, not average-ckpt) \hanchi{for internal only}
% & \textbf{26.0} & 35.2 & \textbf{17.4} & 30.7 & 24.5 & \textbf{23.5} & 29.8 & 28.7 \\

\bottomrule
\end{tabular}}

\caption{Main results on tst-COMMON subset on all 8 languages in MuST-C dataset. ``Speech'' denotes unlabeled audio data. $^\mathsection$: the EN-DE result uses a mixed WMT14+OpenSubtitles data for MT pre-training. Among the baselines, $^\dagger$ shows results from ~\citet{ott2019fairseq}, $^\ddagger$ from ~\citet{inaguma2020espnet}, $^\star$ from ~\citet{zhang2020adaptive}, $^\diamondsuit$ from ~\citet{le2020dual}, $^\sharp$ from ~\citet{liu2020bridging}, $^\flat$ from ~\citet{indurthi2020data}, and $^\circ$ from ~\citet{pino2019harnessing}. $^\ast$ shows results of a simple baseline model by combining a Wav2Vec2 module ~\citep{baevski2020wav2vec} and a Transformer.
% , which could be viewed as the ``no external data'' version of \model.
}
\label{tab:main_results}
\end{table*}

==> arxiv submission v3/tables/memory_size.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Memory Size}
& \multicolumn{2}{c}{EN-DE} & \multicolumn{2}{c}{EN-FR} \\
\cmidrule{2-5}
& MT & ST & MT & ST\\

\midrule
 16 & 30.3 & 25.0 & 43.9 & 34.5 \\
 64 & 32.1 & 25.9 & 46.4 & 35.2 \\
\bottomrule

\end{tabular}
\caption{The influence of different \methodrepresentation sizes on MuST-C tst-COMMON BLEU scores. ``MT'' means transcript-translation performance after MT pretraining, while ``ST'' means the final speech translation scores.}
\label{tab:memory_size}

\end{table}

==> arxiv submission v3/tables/mt_baselines.tex <==
\begin{table}[t!]
\centering
\small
\linespread{1}

\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{lccc|c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{External Data}} 
& \textbf{MuST-C}  \\
& Speech & ASR & MT &  EN-DE \\
\midrule

W2V2-T + Dec PT
& \checkmark & $\times$ & WMT14 & 22.2 \\

W2V2-T + KD
& \checkmark & $\times$ & WMT14 & 24.6\\

\model
& \checkmark & $\times$ & WMT14 & \textbf{26.3}  \\

\bottomrule
\end{tabular}}

\caption{
\cameraready{
Baselines that utilize external MT data. ``Dec PT'' pre-trains decoder on MT corpus; ``KD'' adopts the knowledge distillation technique as ~\citet{liu2019end}
}}
\label{tab:mt_baselines}
\end{table}

==> arxiv submission v3/tables/multitask.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{cc|cc}
\toprule

MT & Contrastive & EN-DE & EN-FR \\ \midrule
 \checkmark & \checkmark & 25.6 & 35.0 \\
 \checkmark & $\times$ & 25.0 & 34.6 \\
 $\times$ & \checkmark & 24.7 & 34.6 \\
 $\times$ & $\times$ & 25.1 & 34.6 \\
 \bottomrule

\end{tabular}
\caption{BLEU scores of Mem-16 \model on MuST-C tst-COMMON set without one or both of auxiliary tasks. ``$\times$'' means this task is not used during fine-tuning, and ``\checkmark'' means othersize. ``Contrastive'' is the bi-modal contrastive task. The removal of one or both of tasks greatly harms the model's performance on both language pairs.}
\label{tab:multitask}

\end{table}

==> body/0443-memory_size.tex <==
\paragraph{\methodrepresentation Length}
% Intuitively, different \methodrepresentation lengths suit different purposes. As source texts are generally shorter than speeches (tens of sub-word tokens versus 50k~1M audio frames), longer memory contains sufficient space for information from speech, while a shorter one prevents over-fitting on MT.
Intuitively, a larger \methodrepresentation length increases the \model's expressive power. We test its effects on two choices of \methodrepresentation lengths: 16 and 64.
% \sout{redundant features}
% \heng{what do you mean by "prevents redundant features"?} 
% \hanchi{How about now?}
% when pretraining on MT. We study the model's behavior by varying the memory length to get quantitative supporting evidence for such hypotheses.
% We tested no two choices of \methodrepresentation lengths: 16 and 64, examining its influence on model performance.
The results are listed in Figure \ref{tab:memory_size}. It shows results on the MuST tst-COMMON set on EN-DE and EN-FR. ``MT'' columns show the transcript-translation BLEUs after MT pretraining. ``ST'' means the final speech translation model. A \methodrepresentation length of 16 generally results in inferior BLEUs on both MT and ST. We hypothesize that this is due to the smaller capacity in \methodrepresentation, which limits its expression ability as well as the amount of knowledge learned during pretraining.

==> body/0444-model_size.tex <==

\paragraph{Model Size}
.
\skeleton{Results are robust against model size changes.}

==> body/050analysis.tex <==
\section{Results and Analysis}
\label{sec:results}

\skeleton{How we could interpret the results presented in \ref{sec:exps}}


% \heng{you should provide more qualitative analysis with examples, and analyze the remaining errors and point out potential solutions.}

==> legacy/000abstract.tex <==
There are common semantics shared across text and images. 
Given a sentence in a source language, whether depicting the visual scene helps translation into a target language?
Existing multimodal neural machine translation methods (MNMT) require triplets of bilingual sentence - image for training and tuples of source sentence - image for inference.
In this paper, we propose \method, a novel machine translation method via visual imagination. 
\method first learns to generate visual representation from the source sentence, and then utilize both source sentence and the ``imagined representation‘’ to produce a target translation.
Unlike previous methods, it only needs the source sentence at the inference time. 
Experiments demonstrate that \method benefits from visual imagination and significantly outperforms the text-only neural machine translation baselines. 
Further analysis reveals that the imagination process in \method  help fill in missing information when performing the degradation strategy. 



% There are thousands of languages on earth, many with distinct characters.
% In contrast, visual illustration can be perceived among peoples. 
% Existing multimodal neural machine translation (MNMT) methods achieve knowledge transfer by enforcing one encoder to learn shared representation across textual and visual modalities. 
% However, these methods rely on well-aligned bilingual sentence - image triplets as the training data and the source sentence - image tuples as the inference input, which are limited in practice. 
% In this paper, we hypothesize that visual imagination via synthesizing visual representation from source text could help the neural model map two languages with different symbols, thus helps the translation task. Our proposed end-to-end imagination-based machine translation model (\method) first learns to generate semantic-consistent visual representation from source sentence, and then generate target sentence based on both text representation and imagined visual representation. Experiments demonstrate that our translation model benefits from visual imagination and significantly outperforms the text-only neural machine translation (NMT) baseline. We also conduct analyzing experiments, and the results show that imagination can help fill in missing information when performing the degradation strategy. 

==> legacy/010intro.tex <==
Visual foundation has been introduced in a novel multimodal Neural Machine Translation (MNMT) task~\citep{specia2016shared,elliott2017findings,barrault2018findings}, which uses bilingual (or multilingual) parallel corpora annotated by images describing sentences' contents (see Figure \ref{fig1}(a)). The superiority of MNMT lies in its ability to use visual information to improve the quality of translation, but its effectiveness largely depends on the availability of data sets, especially the quantity and quality of annotated images. In addition, because the cost of manual image annotation is relatively high, at this stage, MNMT is mostly applied on a small and specific dataset, Multi30K~\cite{elliott2016multi30k}, and is not suitable for large-scale text-only Neural Machine Translation (NMT)~\cite{bahdanau2014neural,vaswani2017attention}. Such limitations hinder the applicability of visual information in NMT.

\begin{figure}[!t]
\centering
\subfigure[Multi-modal NMT]
{
\centering
\includegraphics[width=0.7\columnwidth]{fig/MNMT.pdf}
}
\subfigure[\method]
{
\centering
\includegraphics[width=0.95\columnwidth]{fig/ImagiNMT.pdf}
}
\caption{The problem setup of our proposed \method is different from existing multi-modal NMT. A multi-modal NMT model takes both text and paired image as the input, while \method takes only sentence in the source language as the usual MT task. \method synthesizes an image and utilize the internal visual representation to assist translation. }
\label{fig1}
\end{figure}

%To solve the aforementioned bottlenecks, some proposed to build a lookup table from image dataset, and then use the search-based method to retrieve pictures that match the keywords in the source language. However, the semantic meaning of the entire sentence isn't captured in their model, and the lookup table is built from Multi30K, so the coverage of the pictures is relatively narrow, and the retrieved pictures is not the reconstruction of the entire sentence, containing a lot of irrelevant noise.

To address the bottlenecks mentioned above, \citet{zhang2019neural} propose to build a lookup table from an image dataset and then using the search-based method to retrieve pictures that match the source language keywords. 
However, the lookup table is built from Multi30K, which leads to a relatively limited coverage of the pictures, and potentially  introduce much irrelevant noise. 
It does not always find the exact image corresponding to the text or the image may not even exist in the database. 
\citet{elliott2017imagination} present a multitask learning framework to ground visual representation to a shared space. 
Their architecture called "imagination" shares an encoder between a primary NMT task and an auxiliary task of ranking the visual features for image retrieval. 
However, neither the image is explicitly generated, nor the visual feature is directly leveraged by the translation decoder, the model simply learns the visual grounded shared encoder. Based on other researchers' earlier exploration, we hypothesize that the potential of vision in conventional text-only NMT has not been fully discovered. Instead, we want to explicitly imagine a "vague figure" (see Figure \ref{fig1}(b)) to guide the translation, since \emph{A picture is worth a thousand words}, and imagining the picture of a sentence is the instinctive reaction of a human being who is learning bilingualism.

In this paper, we propose a novel end-to-end machine translation model that is embedded in visual semantics with generative imagination (\method) (see Figure \ref{fig1}(b)). Given a source language sentence, \method first encodes it and transforms the word representations into visual features through an attentive generator, which can effectively capture the semantics of both global and local levels, and the generated visual representations can be considered as semantic-equivalent reconstructions of sentences. A simple yet effective integration module is designed to aggregate the textual and visual modalities. In the final stage, the model learns to generate the target language sentence based on the joint features. To train the model in an end-to-end fashion, we apply a visual realism adversarial loss and a text-image pair-aware adversarial loss, as well as text-semantic reconstruction loss and target language translation loss based on cross-entropy. 

%Furthermore, we also incorporate a triplet ranking loss to make the generated visual feature close to the matched text in the latent visual semantic space.

In contrast with most prior MNMT work, our proposed \method model does not require images as input during the inference time but can leverage visual information through imagination, making it an appealing method in low-resource scenario. Moreover, \method is also flexible, accepting external parallel text data or non-parallel image captioning data. We evaluate our Imagination modal on the Multi30K dataset. The experiment results show that our proposed method significantly outperforms the text-only NMT baseline. The analysis demonstrates that imagination help the model complete the missing information in the sentence when we perform degradation masking, and we also see improvements in translation quality by pre-training the model with an external non-parallel image captioning dataset.

To summarize, the paper has the following contributions: 
\begin{enumerate}
    \item We propose generative imagination, a new setup for machine translation assisted by synthesized visual representation, without annotated images as input;
    \item We propose the \method method, which shows advantages over the conventional MNMT model and gains significant improvements over the text-only NMT baseline;
    \item We conduct experiments to verify and analyze how imagination helps the translation.
\end{enumerate}

==> legacy/020related.tex <==
%Using additional knowledge to construct fine-grained representations is an important issue in language modeling. However, 
\textbf{MNMT}   As a language shared by people worldwide, visual modality may help machines have a more comprehensive perception of the real world. Multimodal neural machine translation (MNMT) is a novel machine translation task proposed by the machine translation community, which aims to design multimodal translation frameworks using context from the additional visual modality \cite{specia2016shared}. The shared task release the dataset Multi30K~\cite{elliott2016multi30k}, which is an extended German version of Flickr30K~\cite{young2014image}, then expanded to French and Czech~\cite{elliott2017findings,barrault2018findings}. In the three versions of tasks, scholars have proposed many multimodal machine translation models and methods. \citet{huang2016attention}  encodes word sequences with regional visual objects, while \citet{calixto2017incorporating} study the effects of incorporating global visual features to initialize the encoder/decoder hidden states of RNN. \citet{caglayan2017lium} models the image-text interaction by leveraging element-wise multiplication. \citet{elliott2017imagination} proposed a multitask learning framework to ground visual representation to a shared space and learn with the auxiliary triplet alignment task. The common practice is to use convolutional neural networks to extract visual information and then using attention mechanisms to extract visual contexts~\cite{caglayan2016multimodal,calixto2016dcu,libovicky2017attention}. \citet{ive2019distilling}  propose a translate-and-refine approach using two-stage decoder. \citet{calixto2018latent} put forward a latent variable model to capture the multimodal interactions between visual and textual features. \citet{caglayan2019probing} show that visual content is more critical when the textual content is limited or uncertain in MMT. Recently, \citet{yao2020multimodal} propose multi-modal self-attention in Transformer to avoid encoding irrelevant information in images, and \citet{yin2020novel} propose a graph-based multimodal fusion encoder to capture various relationships.

%(2) Cross-modal interaction using spatially agnostic global information (\cite{calixto2017incorporating}; \cite{ma2017osu}; \cite{caglayan2017lium}); (3) Regional feature integration from the target detection network (\cite{huang2016attention}; \cite{gronroos2018memad}).

\textbf{Text-to-image synthesis}   Traditional Text-to-image (T2I) synthesis mainly uses keywords to search for small image regions, and finally optimizes the entire layout~\cite{zhu2007text}. After generative adversarial networks (GANs)~\cite{goodfellow2014generative} were proposed, scholars have presented a variety of GAN-based T2I models. \citet{reed2016generative} propose DC-GAN and design a direct and straightforward network and a training strategy for T2I generation. \citet{zhang2017stackgan} propose stackGAN, which contains multiple cascaded generators and discriminators, and the higher stage generates better quality pictures. In previous work, scholars only considered global semantics. \citet{xu2018attngan} proposed AttnGAN to apply the attention mechanism to capture fine-grained word-level information. MirrorGAN~\cite{qiao2019mirrorgan} employs a mirror structure, which reversely learns from the inverse task of T2I to further validate whether generated images are consistent with the input texts. The inverse task is also known as image captioning.

==> legacy/030method.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{fig/model.pdf} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Overview of the framework of the proposed \method. $F_{0}$ and $F_{1}$ are text-to-image converters, comprising of perceptron, residual, and unsampling blocks. L $\times$ represents L identical layers. Noting that we only need to obtain the generated visual feature to guide the translation, up-sampling this feature to image is redundant.}
\label{fig2}
\end{figure*}

As shown in Figure\ref{fig2}, \method embodies the encoder-decoder structure for end-to-end machine translation. Between the encoder and the decoder, there is an imagination step to generate semantic-equivalent visual representation. Technically, our model is composed of following modules: source text encoder, generative imagination network, image captioning, and decoder for translation. We will elaborate on each of them in the rest of this section.

\subsection{Source text encoder}

\citet{vaswani2017attention} propose the state-of-art Transformer-based machine translation framework, which can be written as follows:

\begin{equation}
    \overline{\textbf{H}}^{l}=\textit{LN}(\textit{Att}^{l}(\textbf{Q}^{l-1},\textbf{K}^{l-1},\textbf{V}^{l-1})+\textbf{H}^{l-1}),
\end{equation}

\begin{equation}
    \textbf{H}^{l}=\textit{LN}(\textit{FFN}^{l}(\overline{H}^{l})+\overline{H}^{l}),
\end{equation}

Where $\textit{Att}^{l}$, $\textit{LN}$, and $\textit{FFN}^{l}$ are the self-attention module, layer normalization, and the feed-forward network for the $l$-th identical layer respectively. The core of the Transformer is the multi-head self-attention, in each attention head, we have:

\begin{equation}
    z_{i}=\sum_{j=1}^{n}\alpha_{ij}(x_{j}W^{V}),
\end{equation}

\begin{equation}
    \alpha_{ij}=softmax(\frac{(x_{i}W^{Q})(x_{j}W^{K})^\top }{\sqrt{d}}),
\end{equation}

$W^{V},W^{Q},W^{K}$ are layer-specific trainable parameter matrices. For the output of final stacked layer, we use $w=\{w_{0},w_{1},...,w_{L-1} \}$, $w\in\mathbb{R}^{d\times L}$ to represent the source word embedding, $L$ is the length of the source sentence. Besides, we add a special token to each source language sentence to obtain the sentence representation $s \in \mathbb{R}^{d}$.

\subsection{Generative imagination network}

Generative Adversarial Network~\cite{goodfellow2014generative} has been applied to synthesis images similar to ground truth~\cite{zhang2017stackgan,xu2018attngan,qiao2019mirrorgan}. We follow the common practice of using the conditioning augmentation~\cite{zhang2017stackgan} to enhance robustness to small perturbations along the conditioning text manifold. $F^{ca}$ represents the conditioning augmentation function, and $s^{ca}$ represents the enhanced sentence representation.

\begin{equation}
    s^{ca}=F^{ca}(s),
\end{equation}

$\{F_{0}, F_{1}\}$ are two visual feature converters, including perceptron, residual and upsampling layers. Furthermore, we define $\{f_{0}, f_{1}\}$ are the visual features after two transformations. For detailed layer structure and block design, please refer to ~\cite{xu2018attngan}.

\begin{equation}
    f_{0}=F_{0}(z,s^{ca}),
\end{equation}

\begin{equation}
    f_{1}=F_{1}(f_{0},F^{attn}(f_{0},s^{ca})),
\end{equation}

$z$ is the noise vector, sampled from the standard normal distribution, and it will be concatenated with $s^{ca}$. $f_{0}\in \mathbb{R}^{M_{0}\times N_{0}}$. Each column of $f_{i}$ is a feature vector of a sub-region of the image, which can also be treat as a pseudo-token. To generate fine-grained details at different subregions of the image by paying attention to the relevant words in the source language, we use image vector in each sub-region to query word vectors by leveraging attention strategy. $F^{attn}$ is an attentive function to obtain word-context feature, then we have:

\begin{small}
\begin{equation}
    F^{attn}(f_{0},s^{ca})=\sum _{l=0}^{L-1} (U_{0}w_{l})(softmax(f_{0}^{T}(U_{0}w_{l})))^\top 
\end{equation}
\end{small}


Word feature $w_{l}$ is firstly converted into the common semantic space of the image feature, $U_{0}$ is a perceptron layer. Then it will be multiplied with visual feature $f_{0}$ to acquire the attention score. $f_{1}$ is the output of the imagination network, capturing multiple levels (word level and sentence level) of semantic meaning. It will be utilized directly for target language generation, and it will also be passed to the discriminator for adversarial training.

\subsection{Image captioning}

Image captioning (I2T) can be regarded as the inverse problem of text-to-image generation, generating the given image's description. If an imagined image is semantic equivalent to the source sentence, then its description should be almost identical to the given text. Thus we leverage the image captioning to translate the imagined visual representation back to the source language\cite{qiao2019mirrorgan}, and this symmetric structure can make the imagined visual feature act like a mirror, effectively enhancing the semantic consistency of the imagined visual feature and precisely reflect the underlying semantics. Following \citet{qiao2019mirrorgan}, we utilize the widely used encoder-decoder image captioning framework\cite{vinyals2015show}, and fix the parameter of the pre-trained image captioning framework when end-to-end training other modules in \method.

\begin{equation}
    p_{t}=Decoder(h_{t-1}),t=0,1,...,L-1.
\end{equation}

\begin{equation}
    \mathcal{L}_{I2T} = -\sum_{t=0}^{L-1} \log p_{t}(T_{t}),
    \label{equation10}
\end{equation}

$p_{t}$ is the predicted probability distribution over the words at $t_{0}$-th decoding step, and $T_{t}$ is the $T_{t}$-th entry of the probability vector.

%\subsection{Aligning the VSE space}

%In this section, we align a shared visual-semantic embedding (VSE) space to find a good distributed representation that can capture the semantic meaning across two modalities. Drawing the generated visual representation and the corresponding sentence closer contributes to better semantic alignment in the language latent space, and it can also encourage the imagination network to validate the semantic consistency further.

%Specifically, we leverage the contrastive triplet loss in cross-modal retrieval to encourage the textual-visual alignment in the VSE space~\cite{kiros2014unifying,lee2018stacked}. Furthermore, we utilize fine-grained and bidirectional (textual-to-visual, visual-to-textual) attention mechanisms to learn to value the imagined visual representation with close semantic relatedness to the source sentence. We denote $h^{f}$ to represent object-level visual feature, and $h^{w}$ to represent the token-level textual feature. The visually-attend textual representation $h^{fw}$ is the weighted combination of $h^{w}$. Similarly, $h^{wf}$ represents textually-attend visual representation. For visual-aware attention, we have:

%\begin{equation}
%    h_{j}^{fw} = \sum_{i=0}^{L-1}\alpha_{ij}h_{i}^{w},
%\end{equation}

%\begin{equation}
%    \alpha_{ij}=softmax_{i}(cos(h_{i}^{w},h_{j}^{f})),
%\end{equation}

%Where $j = 0, ..., M-1$. $L$ is the sentence length, and $M$ is the visual feature maps. Then we get:

%\begin{equation}
%\begin{split}
%    S(f,w)=\frac{1}{2M}\sum_{j=0}^{M-1}cos(h_{j}^{fw},h_{j}^{f}) \\
%    +\frac{1}{2L}\sum_{i=0}^{L-1}cos(h_{i}^{wf},h_{i}^{w}) &
%\end{split}
%\end{equation}

%\begin{equation}
%\begin{split}
%    \mathcal{L}_{c}(f,w) = \max_{\Tilde{f}}[\gamma-S(f,w)+S(\Tilde{f},w)]_{+} \\ + \max_{\Tilde{w}}[\gamma-S(f,w)+S(f,\Tilde{w})]_{+} &
%\end{split}
%\end{equation}

%$S(f,w)$ is the cosine similarity between a sentence and an image, $\mathcal{L}_{c}(f,w)$ is the contrastive triplet loss. $\Tilde{f}$ and $\Tilde{w}$ are the contrastive non-paired example with respect to the selected source text and the selected imagined visual representation. $[]_{+}$ is the hinge loss function. When the loss decreases, the distance between a paired image and sentence will drop while the distance between an unpaired image and sentence increases. 

\subsection{Multimodal aggregation}

After obtaining the imagined visual representation, we aggregate two modalities for the translation decoder. Although the vision carries richer information, it also contains irrelevant noise. Comparing to encoding and integrating visual feature directly, a more elegant method is to induce the hidden representation under the guide of image-aware attention and graph perspective of transformer~\cite{yao2020multimodal}, since each local spatial regions of the image can also be considered as pseudo-tokens, which can be added to the source fully-connected graph. In the multimodal self-attention layer, we add the spatial feature of the generated feature map in the source sentence, getting $\Tilde{x}\in\mathbb{R}^{(L+M)\times d}$, then perform image-aware attention, we have:

\begin{equation}
    c_{i}=\sum_{j=0}^{L-1}\Tilde{\alpha}_{ij}(w_{j}W^{V})
\end{equation}

\begin{equation}
    \Tilde{\alpha}_{ij}=softmax(\frac{(\Tilde{x}_{i}W^{Q})(w_{j}W^{K})^\top }{\sqrt{d}})
\end{equation}

\subsection{Objective function}

\begin{figure}[t]
\centering
\includegraphics[width=0.95\columnwidth]{fig/loss1.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Training objective. The discriminator takes source language sentences, generated images, and real images as input, then computes two adversarial loss: realism loss and text-image paired loss. $\mathcal{L}_{I2T}$ is designed to guarantee the semantic consistency, and $\mathcal{L}_{trans}$ is the core loss function to translate integrated embedding to the target language.}
\label{fig3}
\end{figure}

During the translation phase, similar to equation\ref{equation10}, we have:

\begin{equation}
    \mathcal{L}_{trans} = -\sum_{t} \log p_{t}(T_{t})
\end{equation}

To train the whole network end-to-end, we leverage adversarial training to alternatively train the generator and the discriminator. Especially, as shown in Figure\ref{fig3}, the discriminator take the imagined visual representation, source language sentence, and the real image as input, and we employ two adversarial losses: a visual realism adversarial loss, and a text-image pair-aware adversarial loss computed by the discriminator~\cite{zhang2017stackgan,xu2018attngan,qiao2019mirrorgan}. 

\begin{equation}
\begin{split}
        \mathcal{L}_{G_{0}}=-\frac{1}{2}\mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(D(I_{i})]\\ -\frac{1}{2}\mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(D(I_{i},s)]&
\end{split}
\end{equation}

The first term is to distinguish real and fake, ensuring that the generator generates visually realistic images. The second term is to guarantee the semantic consistency between the input text and the generated image. The final objective function of the generator is defined as:

\begin{equation}
    \mathcal{L}_{G}=\mathcal{L}_{G_{0}}+\lambda_{1}\mathcal{L}_{I2T}+ \lambda_{2}\mathcal{L}_{trans}
\end{equation}

Accordingly, the discriminator $D$ is trained by minimizing the following loss:

\begin{equation}
\begin{split}
    L_{D} =-\frac{1}{2} \mathbb{E}_{I_{i}^{GT}\sim p_{I_{i}^{G}}}[\log(D(I_{i}^{GT})]\\
    -\frac{1}{2} \mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(1-(I_{i})] \\
    -\frac{1}{2} \mathbb{E}_{I_{i}^{GT}\sim p_{I_{i}^{G}}}[\log(D(I_{i}^{GT},s)]\\
    -\frac{1}{2} \mathbb{E}_{I_{i}\sim p_{I_{i}}}[\log(1-D(I_{i},s)]&
\end{split}
\end{equation}

==> legacy/040experiment.tex <==
\subsection{Datasets}

\begin{table*}[ht]
\centering
\small
\linespread{1.2}
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{l|cccccc}
\hline
\multirow{3}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{En$\Rightarrow$De}}  \\
\cline{2-7}
& \multicolumn{2}{c}{\textbf{Test2016}}  
& \multicolumn{2}{c}{\textbf{Test2017}} 
& \multicolumn{2}{c}{\textbf{Ambiguous COCO}} \\
\cline{2-7}
& BLEU & METEOR & BLEU & METEOR & BLEU & METEOR \\
\hline
\hline
\multicolumn{7}{c}{\emph{Multimodal Neural Machine Translation Systems}} \\
\hline
IMG$_{D}$ ~\cite{calixto2017incorporating} & 37.3 & 55.1 & N/A & N/A & N/A & N/A \\
NMT$_{SRC+IMG}$ ~\cite{calixto2017doubly}  & 36.5 & 55.0 & N/A & N/A & N/A & N/A  \\
trg-mul ~\cite{caglayan2017lium} & 37.8 & \textbf{57.7} & 30.7 & 52.2 & 27.1 & 47.2 \\
VAG-NMT ~\cite{zhou2018visual} & N/A & N/A & 31.6 & 52.2 & 28.3 & 48.0 \\
Transformer+Att ~\cite{ive2019distilling} & 38.0 & 55.6 & N/A & N/A & N/A & N/A \\
Multimodal transformer ~\cite{yao2020multimodal} & 38.7 & 55.7 & N/A & N/A & N/A & N/A \\
\method + ground truth & 38.6 & 55.7 & 32.4 & 52.5 & 28.8 & 48.9 \\
\hline
\multicolumn{7}{c}{\emph{Text-only Neural Machine Translation Systems}} \\
\hline
Transformer baseline ~\cite{vaswani2017attention} & 37.6 & 55.3 & 31.7 & 52.1 & 27.9 & 47.8 \\
Multitask ~\cite{elliott2017imagination} & 36.8 & 55.8 & 30.2 & 51.2 & N/A & N/A \\
VMMT$_{F}$~\cite{calixto2018latent} & 37.6 & 56.0 & N/A & N/A & N/A & N/A \\
Lookup table ~\cite{zhang2019neural} & 36.9 & N/A & 28.6 & N/A & N/A & N/A \\
\method & 38.5 & 55.7 & 32.1 & 52.4 & 28.7 & 48.8 \\
\hline
\end{tabular}}
\caption{Main result from the Test2016, Test2017, and Ambiguous COCO for the En$\Rightarrow$De MNMT task. The first category collects the existing MNMT systems, which take both source sentences and paired images as input. The second category illustrates the systems that do not require images as input. Since our method falls into the second group, our baseline are the text-only transformer~\cite{vaswani2017attention} and the aforementioned works~\cite{zhang2019neural,elliott2017imagination}.}
\label{Table_En2DeMainResults}
\end{table*}

We evaluate our proposed \method model on two datasets, Multi30K~\cite{elliott2016multi30k} and Ambiguous COCO~\cite{elliott2017findings}. To show its ability to train with external out-of-domain datasets, we adopt MS COCO~\cite{lin2014microsoft} in the next analyzing section.

Multi30K is the largest existing human-labeled collection for MNMT, containing $31K$ images and consisting of two multilingual expansions of the original Flickr30K\cite{young2014image} dataset. The first expansion has five English descriptions and five German descriptions, and they are independent of each other. The second expansion has one of its English description manually translated to German by a professional translator, then expanded to French and Czech in the following shared task~\cite{elliott2017findings,barrault2018findings}. We only apply the second expansion in our experiments, which has $29,000$ instances for training, $1,014$ for development, and $1,000$ for evaluation. We present our results on English-German (En-De) Test2016 and Test2017.

Ambiguous COCO is a small evaluation dataset collected in the WMT2017 multimodal machine translation challenge~\cite{elliott2017findings}, which collected and translated a set of image descriptions that potentially contain ambiguous verbs. It contains $461$ images from the MS COCO\cite{lin2014microsoft} for $56$ ambiguous vers in total. 

MS COCO is the widely used non-parallel text-image paired dataset in T2I and I2T generation. It contains $82,783$ training images and $40,504$ validation images with $91$ different object types, and each image has 5 English descriptions.

\subsection{Settings}

Our baseline is the conventional text-only Transformer~\cite{vaswani2017attention}. Specifically, each encoder-decoder has a 6-layer stacked Transformer network, eight heads, 512 hidden units, and the inner feed-forward layer filter size is set to 2048. The dropout is set to $p=0.1$, and we use Adam optimizer~\cite{kingma2014adam} to tune the parameter. The learning rate increases linearly for the warmup strategy with $8,000$ steps and decreases with the step number's inverse square root. We train the model up to $10,000$ steps, the early-stop strategy is adopted. We use the same setting as \citet{vaswani2017attention}. We use the metrics BLEU~\cite{papineni-etal-2002-bleu} and METEOR~\cite{denkowski-lavie-2014-meteor}to evaluate the translation quality.

For the imagination network, the noise vector's dimension is $100$, and the generated visual feature is $128\times128$. The upsampling and residual block in visual feature transformers consist of $3\times3$ stride 1 convolution, batch normalization, and ReLU activation. The training is early-stopped if the dev set BLEU score do not improve for $10$ epochs, since the translation is the core task. The batch size is $64$, and the learning rate is initialized to be $2e^{-4}$ and decayed to half of its previous value every $100$ epochs. A similar learning schedule is adopted in \citet{zhang2017stackgan}. The margin size $\gamma$ is set to $0.1$, the balance weight $\lambda_{1}=20$, $\lambda_{2}=40$. 

\subsection{Results}

Table \ref{Table_En2DeMainResults} illustrates the results for the Test2016, Test2017, and the Ambiguous COCO MNMT tasks. Our text-only Transformer baseline~\cite{vaswani2017attention} has similar results compared to most prior MNMT works, which is consistent with the previous findings~\cite{caglayan2019probing}, that is, textual modality is good enough to translate for Multi30K dataset. This finding helps to explain that it is already tricky for a MNMT model to ground visual modality even with the presence of annotated images. However, Our \method gains improvements over the text-only Transformer baseline on three evaluation datasets, demonstrating that our model can effectively embed the visual semantics during the training time and guide the translation through imagination with the absence of annotated images during the inference time. We assume much of the performance improvement is due to \method's strong ability to capture the interaction between text and image, generate semantic-consistent visual representations, and incorporate information from visual modality properly. 

We also observe that our approach surpasses the results of most MNMT systems by a noticeable margin in terms of BLEU score and METEOR score on three evaluation dataset. Our \method is also competitive with \method + ground truth, which is our translation decoder taking ground truth visual representations instead of imagined ones. This proves imaginative ability of \method.

For Ambiguous COCO, which was purposely curated such that verbs have ambiguous meaning, demands more visual contribution for guiding the translation and selecting correct words. Our \method benefits from visual imagination and substantially outperforms previous works on ambiguous COCO.

\subsection{Ablation studies}

\begin{table}[ht]
\centering
\begin{tabular}{l|cc}
\hline
 Evaluation metric             & BLEU   & METEOR     \\ \hline
 ImagiT, $\lambda_{1}=0$ & 37.9 & 55.3 \\ \hline
  ImagiT, $\lambda_{1}=5$ & 38.2 & 55.5 \\ \hline
   ImagiT, $\lambda_{1}=10$ & 38.4 & 55.7 \\ \hline
    ImagiT, $\lambda_{1}=20$ & 38.5 & 55.7 \\ \hline
     ImagiT, $\lambda_{1}=40$ & 38.3 & 55.6 \\ \hline
\end{tabular}
\caption{Ablation studies of ImagiT with different weight settings}
\label{table2}
\end{table}

The hyper-parameter $\lambda_{1}$ is important. When $\lambda_{1}=0$, there is no image captioning component, the BLEU score drops from 38.6 to 37.9, while this variant still outperforms the Transformer baseline. This indicates the effectiveness of image captioning module, since it will potentially prevent visual-textual mismatching, thus helps generator achieve better performance. When $\lambda_{1}$ increases from $5$ to $20$, the BLEU and METEOR increase accordingly. Whereas $\lambda_{1}$ is set to equal to $\lambda_{2}$ ($40$), the BLEU score falls to 38.4. That's reasonable because $\lambda_{2}\mathcal{L}_{trans}$ is the main task of the whole model.

==> legacy/050analyse.tex <==
\subsection{Can \method generate visual grounded representations?}

Since the proposed model does not require images as input, one may ask how it uses visual information and where the information comes? We claim that \method has already been embedded with visual semantics during the training phase, and in this section, we validate that \method is able to generate visual grounded representation by performing the image retrieval task.

For each source sentence, we generate the intermediate visual representation. Furthermore, we query the ground truth image features for each generated representation to find the closest image vectors around it based on the cosine similarity. Then we can measure the $R@K$ score, which computes the recall rate of the matched image in the top K nearest neighborhoods.

\begin{table}[h]
\centering
\begin{tabular}{l|ccc}
\hline
              & $R@1$     & $R@5$ &  $R@10$   \\ \hline
\method on Multi30K & 64.7  & 88.7 & 94.2 \\ \hline
\method on MS COCO & 64.3  &  89.5   & 94.7 \\
\hline
\end{tabular}
\caption{Image retrieval task. We evaluate on Multi30K and MS COCO.}
\label{retrieval}
\end{table}

Some previous studies on VSE perform sentence-to-image retrieval and image-to-sentence retrieval, but their results can not be directly compared with ours, since we are performing image-to-image retrieval in practical. However, from Table \ref{retrieval}, especially for $R@10$, the results demonstrate that our generated representation has excellent quality of shared semantics and have been grounded with visual semantic-consistency. 

\subsection{How does the imagination help the translation?}

Although we have validated the effectiveness of \method on three widely used MNMT evaluation datasets. A natural question to ask is that how does the imagination guide the translation, and to which extent? When human beings confronting with complicate sentences and obscure words, we often resort to mind-picturing and mental visualization to assist us to auto-complete and fill the whole imagination. Thus we hypothesis that imagination could help recover and retrieve the missing and implicate textual information.

Inspired by \citet{ive2019distilling,caglayan2019probing}, we apply degradation strategy to the input source language, and feed to the trained Transformer baseline, MNMT baseline, and \method respectively, to validate if our proposed approach could recover the missing information and obtain better performance. And we conduct the analysing experiments on En-De Test2016 evaluation set.

\textbf{Color deprivation} is to mask the source tokens that refers to colors, and replace them with a special token [M]. Under this circumstance, text-only NMT model have to rely on source-side contextual information and biases, while for MNMT model, it can directly utilize the paired color-related information-rich images. But for \method, the model will turn to imagination and visualization.

\begin{table}[!h]
\centering
\begin{tabular}{l|cc}
\hline
 Model             & $S$     & $\overline{S}$    \\ \hline
text-only Transformer & 37.6  & 36.3 \\ \hline
MNMT        & 38.2 & 37.7 \\ \hline
\method       & 38.4 & 37.9 \\
\hline
\end{tabular}
\caption{Color deprivation. $s$ represents the original source sentence, while $\overline{s}$ is the degraded sentence.}
\label{color deprivation}
\end{table}

Table ~\ref{color deprivation} demonstrates the results of color deprivation. We implement a simple transformer-based MNMT baseline model using the multimodal self-attention approach~\cite{yao2020multimodal}. Thus the illustrated three models in Table\ref{table2} can be compared directly. We can observe that the BLEU score of text-only NMT decreases 1.3, whereas MNMT and \method system only decreases 0.5. This result corroborates that our \method has a similar ability to recover color compared to MNMT, but our \method achieves the same effect through its own efforts, i.e., imagination.

\textbf{Visually depictable entity masking}. \citet{plummer2015flickr30k} extend Flickr30K with cereference chains to tag mentions of visually depictable entities. Similar to color deprivation, we randomly replace $0\%,15\%,30\%,45\%,60\%$ visually depictable entities with a special token [M].

\begin{figure}[h]
\centering
\includegraphics[width=0.95\columnwidth]{fig/analyse.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Visually depictable entity masking. From top to bottom is MNMT, \method, text-only transformer.}
\label{fig4}
\end{figure}

Figure~\ref{fig4} is the result of visually depictable entity masking. We observe a large BLEU score drop of text-only Transformer baseline with the increasing of masking proportion, while MNMT and \method are relatively smaller. This result demonstrates that our \method model can much more effectively infer and imagine missing entities compared to text-only Transformer, and have comparable capability over the MNMT model.

\subsection{Will better imagination with external data render better translation?}

Our \method model also accepts external parallel text data or non-parallel image captioning data, and we can easily modify the objective function to train with out-of-domain non-triple data. To train with text-image paired image captioning data, we can pre-train our imagination model by ignoring $\mathcal{L}_{trans}$ term. In other words, the T2I synthesis module can be solely trained with MS COCO dataset. We randomly split MS COCO in half, and use COCO$_{half}$ and COCO$_{full}$ to pre-train \method. The MS COCO is processed using the same pipeline as in \citet{zhang2017stackgan}. Furthermore, the training setting of COCO$_{half}$ and COCO$_{full}$ are the same with batch size $64$ and maximum epoch $600$. The results are:

\begin{table}[!h]
\centering
\begin{tabular}{l|cc}
\hline
              & BLEU     & METEOR    \\ \hline
\method & 38.4  & 55.7 \\ \hline
\method + COCO$_{half}$& 38.6 & 56.3 \\ \hline
\method + COCO$_{full}$& 38.7 & 56.7 \\
\hline
\end{tabular}
\caption{Translation results when using out-of-domain non-parallel image captioning data.}
\label{table3}
\end{table}

As is shown in Table\ref{table3}, our \method model pre-trained with half MS COCO gain 0.6 METEOR increase, and the improvement becomes more apparent when training with the whole MS COCO. We can contemplate that large-scale external data may further improve the performance of \method, and we have not utilized parallel text data (e.g., WMT), even image-only and monolingual text data can also be adopted to enhance the model capability, and we leave this for future work.

==> legacy/060conclusion.tex <==
This work presents generative imagination-based machine translation model (\method), which can effectively capture the source semantics and generate semantic-consistent visual representations for imagination-guided translation. Without annotated images as input, out model gains significant improvements over text-only NMT baselines and is comparable with the SOTA MNMT model. We analyze how imagination elevates machine translation and show improvement using external image captioning data. Further work may center around introducing more parallel and non-parallel, text, and image data for different training schemes. 

==> tables/contrastive_ablation.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{l|cc}
\toprule

 
Language & with & w/o \\
\midrule
EN-DE & 24.5 & 24.4 \\
EN-FR & 34.5 & 33.7 \\
EN-RU & 16.6 & 16.4 \\
EN-ES & 30.0 & 29.9 \\
\bottomrule

\end{tabular}
\caption{BLEU scores of \model on MuST-C tst-COMMON set with (``with'') or without (``w/o'') dual-modal contrastive trainig. Result on EN-FR shows the largest drop, proving it more necessary to align between speech and text representations for \model when MT pretraining data is larger.}
\label{tab:contrastive_ablation}

\end{table}

==> tables/memory_size.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{c|cccc}
\toprule

\multirow{2}{*}{Memory Size}
& \multicolumn{2}{c}{EN-DE} & \multicolumn{2}{c}{EN-FR} \\
\cmidrule{2-5}
& MT & ST & MT & ST\\

\midrule
 16 & 30.3 & 25.0 & 43.9 & 34.5 \\
 64 & 32.1 & 25.9 & 46.4 & 35.2 \\
\bottomrule

\end{tabular}
\caption{The influence of different \methodrepresentation sizes on MuST-C tst-COMMON BLEU scores. ``MT'' means transcript-translation performance after MT pretraining, while ``ST'' means the final speech translation scores.}
\label{tab:memory_size}

\end{table}
